Computational Performance of a LES Solver for Supersonic Jet Flow Applications

An in-house large eddy simulation tool is developed in order to reproduce high fidelity results of compressible jet flows. The large eddy simulation formulation is written using the finite difference approach, with an explicit time integration and using a second order spatial discretization. The energy equation is carefully discretized in order to model the energy equation of the filtered Navier-Stokes formulation. Such nu\-me\-ri\-cal studies are very expensive and demand high performance computing. Message passage interface protocols are implemented into the code in order to perform parallel computations. The present work addresses the computational performance of the solver running on up to 400 processors in parallel. Different mesh configurations, whose size varies from approximately 5.9 million points to approximately 1.0 billion points, are evaluate in the current paper. Speedup and efficiency curves are evaluated in order to assess the strong scalability of the solver.

==> sources/abstract.tex <==
\section*{Abstract}

New acoustics design constraints have ecouraged the 
studies of aeroacoustics fields around compressible jet 
flows. Instituto de Aeron\'{a}utica e Espa\c{c}o (IAE) 
in Brazil is interested in this flow configuration for rocket 
design applications. Therefore, the current work addresses 
the numerical study of unsteady turbulent 
flows for aeroacoustic applications of the Brazilian 
institute. A novel large eddy simulation tool is 
developed in order to reproduce high fidelity results 
of compressible jet flows which are used for aeroacoustic 
studies using the Ffowcs Williams and Hawkingg approach. 
The numerical solver is an upgrade of a Reynolds-averaged 
Navier-Stokes developed by the Brazilian research group. 
Generally, large eddy simulations demands very refined meshes. 
Hence, high performance computing is a requirement for such 
simulations. Therefore, the original framework is rewritten 
in a modern fashion and parallel computation capabilities have 
been added to the code. The communication between processors are 
performed by message passing interface protocols. The CFD 
general notation system is also included in the numerical 
tool. The large eddy simulation formulation is written using 
the finite difference approach. Inviscid numerical fluxes are 
calculated using a second-order accurate centered scheme with 
the explicit addition of artificial dissipation. A five steps 
second-order accurate Runge-Kutta is the chosen time marching 
method. The energy equation is carefully discretized in order 
to model the energy equation of the filtered Navier Stokes 
formulation. The classical Smagorinsky model is the chosen 
turbulence closure for the present work. Numerical simulation 
of a perfectly expanded jet are being performed and compared with
the literature in order to validate the new solver. Moreover, 
the speedup and the computational performance of the code are 
evaluated and dicussed.


==> sources/annex/annex_a.tex <==
\chapter{Subgrid Tensor}

\begin{eqnarray}
L_{ij} = - \overline{\rho} \left( \, \langle {\langle u_{i} \rangle \langle u_{j} \rangle} \rangle 
- \langle u_{i} \rangle \langle u_{j} \rangle \, \right)
& \rightarrow & \mbox{Leonard tensor} \nonumber \\
C_{ij} =  - \overline{\rho} \left( \, \langle {\langle u_{i} \rangle u_{j}''} \rangle
+ \langle {\langle u_{j} \rangle u_{i}''} \rangle \, \right)
& \rightarrow & \mbox{Clarck tensor} \\
R_{ij} = - \overline{\rho} \langle {u_{j}'' u_{i}''} \rangle
& \rightarrow & \mbox{Reynolds tensor} \nonumber
\end{eqnarray}

Bardina simirality
%
\begin{equation}
\langle \phi \psi \rangle \approx \langle \phi \rangle \langle \psi \rangle
\end{equation}

using
%
\begin{equation}
u = \langle u \rangle + u''
\end{equation}

one can write
%
\begin{eqnarray}
C_{ij} & = &  - \overline{\rho} \left\{ \, \langle \left[ {\langle u_{i} \rangle \left( u_{j} - \langle u_{j} \rangle  \right)} \right] \rangle
+ \langle \left[ { \left( u_{i} - \langle u_{i} \rangle  \right)  \langle u_{j} \rangle} \right] \rangle \, \right\} \nonumber\\
& = &  - \overline{\rho} \left[ \, \langle \langle u_{i} \rangle  \rangle \, \langle u_{j} - \langle u_{j} \rangle \rangle
+ \langle u_{i} - \langle u_{i} \rangle \rangle \langle \langle u_{j} \rangle \rangle \, \right] \nonumber\\
& = &  - \overline{\rho} \left[ \, \langle \langle u_{i} \rangle \rangle \, \left( \langle u_{j} \rangle - \langle \langle u_{j} \rangle \rangle \right)
+ \left( \langle u_{i} \rangle - \langle \langle u_{i} \rangle \rangle \right) \, \langle \langle u_{j} \rangle \rangle \, \right] \nonumber\\
C_{ij} & = &  - \overline{\rho} \left[ \, \langle \langle u_{i} \rangle \rangle \langle u_{j} \rangle - \langle \langle u_{i} \rangle \rangle \langle \langle u_{j} \rangle \rangle
+ \langle u_{i} \rangle \langle \langle u_{j} \rangle \rangle - \langle \langle u_{i} \rangle \langle \langle u_{j} \rangle \rangle \, \right] 
\end{eqnarray}
%
and
%
\begin{eqnarray}
R_{ij} & = & - \overline{\rho} \langle \left[ \left( u_{i} - \langle u_{i} \rangle \right)  \left( u_{j} - \langle u_{j} \rangle \right) \right] \rangle \nonumber \\
 & = & - \overline{\rho} \left[ \langle u_{i} - \langle u_{i} \rangle \rangle  \langle u_{j} - \langle u_{j} \rangle \rangle \right] \nonumber \\
 & = & - \overline{\rho} \left[ \left( \langle u_{i} \rangle - \langle \langle u_{i} \rangle \rangle \right) \left( \langle u_{j} \rangle - \langle \langle u_{j} \rangle \rangle \right) \right] \nonumber \\
R_{ij} & = & - \overline{\rho} \left[ \langle u_{i} \rangle \langle u_{j} \rangle - \langle u_{i} \rangle \langle \langle u_{j} \rangle \rangle
- \langle \langle u_{i} \rangle \rangle \langle u_{j} \rangle + \langle \langle u_{i} \rangle \rangle \langle \langle u_{j} \rangle \rangle \right] 
\end{eqnarray}
%
\begin{equation}
\sigma_{ij} = L_{ij} + C_{ij} + R_{ij}
\end{equation}
%
\begin{eqnarray}
\sigma_{ij} & = & - \overline{\rho} \left[ \langle { \langle u_{i} \rangle \langle u_{j} \rangle} \rangle 
- \langle u_{i} \rangle \langle u_{j} \rangle \right] \nonumber \\
& &  - \overline{\rho} \left[ \langle \langle u_{i} \rangle \rangle \langle u_{j} \rangle - \langle \langle u_{i} \rangle \rangle \langle \langle u_{j} \rangle \rangle
+ \langle u_{i} \rangle \langle \langle u_{j} \rangle \rangle - \langle \langle u_{i} \rangle \langle \langle u_{j} \rangle \rangle \right] \nonumber \\
& & - \overline{\rho} \left[ \langle u_{i} \rangle \langle u_{j} \rangle - \langle u_{i} \rangle \langle \langle u_{j} \rangle \rangle
- \langle \langle u_{i} \rangle \rangle \langle u_{j} \rangle + \langle \langle u_{i} \rangle \rangle \langle \langle u_{j} \rangle \rangle \right] 
\end{eqnarray}
%
and then
%
\begin{equation}
\sigma_{ij} = -\overline{\rho} \left[ \langle \langle u_{i} \rangle \langle u_{j} \rangle \rangle  - \langle \langle u_{i} \rangle \rangle \langle \langle u_{j} \rangle \rangle \right]
\end{equation}


==> sources/conclusion/conclusion.tex <==
%\section{Concluding Remarks}
%
%The current work is the study on effects of different 
%subgrid scales models on perfectly expanded supersonic jet 
%flow configurations using centered second-order spatial 
%discratization. A formulation based on the the System I set 
%of equations is used in the present work. The time integration 
%is performed using a five-steps second order Runge-Kutta scheme.
%Four large eddy simulations of compressible jet flows are performed 
%in the present research using two different mesh configurations 
%an three different subgrid scale models. Their effects
%on the large eddy simulation solution are compared and discussed.
%
%The mesh refinement study has indicated that in the region 
%where the grid presents high resolution, the simulations
%are in good agreement with experimental and numerical 
%references. For the mesh with 14 million points the simulation 
%has produced good results for $X<2.5D$ and $-1.5D<Y<0.5D$.
%For the other mesh, with 50 million points, the simulations
%provided good agreement with the literature for $X<5.0D$ and 
%$-1.5D<Y<0.5D$. The eddy viscosity, calculated by the static
%Smagorinsky model, presents very low levels in the region 
%where the results have good correlation with the results of
%the literature.
%
%The refined grid used on the mesh refinement study, mesh B,
%is used for the comparison of SGS models effects on the 
%results of large eddy simulations. Three compressible jet
%flow simulations are performed using the classic Smagorinsky
%model \cite{Smagorinsky63,Lilly65,Lilly67}, the dynamic 
%Smagorinsky model \cite{Germano91,moin91} and the Vreman model
%\cite{vreman2004}. All three simulations presented similar 
%behavior. Results presented good agreement with the reference 
%for $X<5.0D$. In the region where the grid is very fine and 
%the results correlates well with the literature, the eddy 
%viscosity, provided by the SGS model, is very low values. 
%The reason is related to the fact that the SGS closures used 
%in the current work are strongly dependent of the filter width, 
%which is proportional to the local mesh size. 
%
%The numerical results indicated that it is possible to achieve
%good results using second-order spatial discetization. The
%mesh ought be well resolved in order to overcome the truncation 
%errors from the low order numerical scheme. Very fine meshes 
%originates very small filter width. Consequently, the effects 
%of the eddy viscosity calculated by the SGS models on the
%solution become unimportant. The work of Li and Wang \cite{Li15} 
%have presented simular conclusions for simplified problems.
%The authors indicate that SGS closures introduce numerical 
%dissipation that can be used as a stabilizing mechaninsm. 
%However, this numerical dissipation does not necessarily add 
%more physics of the turbulence to the LES solution. Simulations 
%without the use of any SGS model are welcome and could reinforce 
%the argument.
%


==> sources/coord/coord.tex <==
\section{Transformation of Coordinates}

The legacy code formulation \cite{BIGA02} was originally written in the a general curvilinear coordinate 
system in order to facilitate the implementation and add more generality for the CFD tool. This approach is 
kept in the present LES solver for the simulation of compressible jet flows. Hence, the filtered Navier-Stokes 
equations can be written in strong conservation form for a 3-D general curvilinear coordinate system as
%
\begin{equation}
	\frac{\partial \hat{Q}}{\partial \mathcal{T}} 
	+ \frac{\partial }{\partial \xi}\left(\hat{\mathbf{E}_{e}}-\hat{\mathbf{E}_{v}}\right) 
	+ \frac{\partial}{\partial \eta}\left(\hat{\mathbf{F}_{e}}-\hat{\mathbf{F}_{v}}\right)
	+ \frac{\partial}{\partial \zeta}\left(\hat{\mathbf{G}_{e}}-\hat{\mathbf{G}_{v}}\right) 
	= 0 \, \mbox{.}
	\label{eq:vec-LES}
\end{equation}
%
In the present work, the chosen general coordinate transformation is given by
%
\begin{eqnarray}
	\mathcal{T} & = & t \, \mbox{,} \nonumber\\
	\xi & = & \xi \left(x,y,z,t \right)  \, \mbox{,} \nonumber\\
	\eta & = & \eta \left(x,y,z,t \right)  \, \mbox{,} \\
	\zeta & = & \zeta \left(x,y,z,t \right)\ \, \mbox{.} \nonumber
\end{eqnarray}
%
In the jet flow configuration, $\xi$ is the axial jet flow direction, $\eta$ is 
the radial direction and $\zeta$ is the azimuthal direction. The vector of
conserved properties is written as
%
\begin{equation}
	\hat{Q} = J^{-1} \left[ \overline{\rho} \quad \overline{\rho}\tilde{u} \quad 
	\overline{\rho}\tilde{v} \quad \overline{\rho}\tilde{w} \quad \overline{e} \right]^{T} 
	\quad \mbox{,}
	\label{eq:hat_Q_vec}
\end{equation}
%
where the Jacobian of the transformation, $J$, is given by
%
\begin{equation}
	J = \left( x_{\xi} y_{\eta} z_{\zeta} + x_{\eta}y_{\zeta}z_{\xi} +
	           x_{\zeta} y_{\xi} z_{\eta} - x_{\xi}y_{\zeta}z_{\eta} -
			   x_{\eta} y_{\xi} z_{\zeta} - x_{\zeta}y_{\eta}z_{\xi} 
	    \right)^{-1} \, \mbox{,}
\end{equation}
%
and
%
\begin{eqnarray}
	\displaystyle x_{\xi}   = \frac{\partial x}{\partial \xi}  \, \mbox{,} & 
	\displaystyle x_{\eta}  = \frac{\partial x}{\partial \eta} \, \mbox{,} & 
	\displaystyle x_{\zeta} = \frac{\partial x}{\partial \zeta}\, \mbox{,} \nonumber \\
	\displaystyle y_{\xi}   = \frac{\partial y}{\partial \xi}  \, \mbox{,} & 
	\displaystyle y_{\eta}  = \frac{\partial y}{\partial \eta} \, \mbox{,} & 
	\displaystyle y_{\zeta} = \frac{\partial y}{\partial \zeta}\, \mbox{,} \\
	\displaystyle z_{\xi}   = \frac{\partial z}{\partial \xi}  \, \mbox{,} & 
	\displaystyle z_{\eta}  = \frac{\partial z}{\partial \eta} \, \mbox{,} & 
	\displaystyle z_{\zeta} = \frac{\partial z}{\partial \zeta}\, \mbox{.} \nonumber
\end{eqnarray}
%

The inviscid flux vectors, $\hat{\mathbf{E}}_{e}$, $\hat{\mathbf{F}}_{e}$ and 
$\hat{\mathbf{G}}_{e}$, are given by
%
{\small
\begin{eqnarray}
	\hat{\mathbf{E}}_{e} = J^{-1} \left\{\begin{array}{c}
		\overline{\rho} U \\
		\overline{\rho}\tilde{u} U + \overline{p} \xi_{x} \\
		\overline{\rho}\tilde{v} U + \overline{p} \xi_{y} \\
		\overline{\rho}\tilde{w} U + \overline{p} \xi_{z} \\
		\left( \overline{e} + \overline{p} \right) U - \overline{p} \xi_{t}
\end{array}\right\} \, \mbox{,} &
%	\label{eq:hat-flux-E}
%\end{equation}
%
%\begin{equation}
	\hat{\mathbf{F}}_{e} = J^{-1} \left\{\begin{array}{c}
		\overline{\rho} V \\
		\overline{\rho}\tilde{u} V + \overline{p} \eta_{x} \\
		\overline{\rho}\tilde{v} V + \overline{p} \eta_{y} \\
		\overline{\rho}\tilde{w} V + \overline{p} \eta_{z} \\
		\left( \overline{e} + \overline{p} \right) V - \overline{p} \eta_{t}
\end{array}\right\} \, \mbox{,} &
%	\label{eq:hat-flux-F}
%\end{equation}
%
%\begin{equation}
	\hat{\mathbf{G}}_{e} = J^{-1} \left\{\begin{array}{c}
		\overline{\rho} W \\
		\overline{\rho}\tilde{u} W + \overline{p} \zeta_{x} \\
		\overline{\rho}\tilde{v} W + \overline{p} \zeta_{y} \\
		\overline{\rho}\tilde{w} W + \overline{p} \zeta_{z} \\
		\left( \overline{e} + \overline{p} \right) W - \overline{p} \zeta_{t}
	\end{array}\right\} \, \mbox{.}
	\label{eq:hat-flux-G}
\end{eqnarray}
}
%
The contravariant velocity components, $U$, $V$ and $W$, are calculated as
%
\begin{eqnarray}
  U = \xi_{t} + \xi_{x}\overline{u} + \xi_{y}\overline{v} + \xi_{z}\overline{w} 
  \, \mbox{,} \nonumber \\
  V = \eta_{t} + \eta_{x}\overline{u} + \eta_{y}\overline{v} + \eta_{z}\overline{w} 
  \, \mbox{,} \\
  W = \zeta_{t} + \zeta_{x}\overline{u} + \zeta_{y}\overline{v} + \zeta_{z}\overline{w} 
  \, \mbox{.} \nonumber
  \label{eq:vel_contrv}
\end{eqnarray}
%
The metric terms are given by
%
\begin{eqnarray}
	\xi_{x} = J \left( y_{\eta}z_{\zeta} - y_{\zeta}z_{\eta} \right) \, \mbox{,} & 
	\xi_{y} = J \left( z_{\eta}x_{\zeta} - z_{\zeta}x_{\eta} \right) \, \mbox{,} & 
	\xi_{z} = J \left( x_{\eta}y_{\zeta} - x_{\zeta}y_{\eta} \right) \, \mbox{,} \nonumber \\
	\eta_{x} = J \left( y_{\eta}z_{\xi} - y_{\xi}z_{\eta} \right) \, \mbox{,} & 
	\eta_{y} = J \left( z_{\eta}x_{\xi} - z_{\xi}x_{\eta} \right) \, \mbox{,} & 
	\eta_{z} = J \left( x_{\eta}y_{\xi} - x_{\xi}y_{\eta} \right) \, \mbox{,} \\
	\zeta_{x} = J \left( y_{\xi}z_{\eta} - y_{\eta}z_{\xi} \right) \, \mbox{,} & 
	\zeta_{y} = J \left( z_{\xi}x_{\eta} - z_{\eta}x_{\xi} \right) \, \mbox{,} & 
	\zeta_{z} = J \left( x_{\xi}y_{\eta} - x_{\eta}y_{\xi} \right) \, \mbox{,} \nonumber \\
	\xi_{t} = -x_{\mathcal{T}}\xi_{x} - y_{\mathcal{T}}\xi_{y} - z_{\mathcal{T}}\xi_{z} \, \mbox{,} & 
	\eta_{t} = -x_{\mathcal{T}}\eta_{x} - y_{\mathcal{T}}\eta_{y} - z_{\mathcal{T}}\eta_{z} \, \mbox{,} & 
	\zeta_{t} = -x_{\mathcal{T}}\zeta_{x} - y_{\mathcal{T}}\zeta_{y} - z_{\mathcal{T}}\zeta_{z} \, \mbox{.} 
	\nonumber
%	\xi_{t} = -x_{\mathcal{T}}\xi_{x} - y_{\mathcal{T}}\xi_{y}  \, \mbox{,} & 
%	\eta_{t} = -x_{\mathcal{T}}\eta_{x} - y_{\mathcal{T}}\eta_{y}  \, \mbox{,} & 
%	\zeta_{t} = -x_{\mathcal{T}}\zeta_{x} - y_{\mathcal{T}}\zeta_{y}  \, \mbox{.} \nonumber \\ 
%	- z_{\mathcal{T}}\xi_{z} & - z_{\mathcal{T}}\eta_{z} & - z_{\mathcal{T}}\zeta_{z}  \nonumber
\end{eqnarray}
%
%One can rewrite Eq.\ \eqref{eq:vec-RANS}, in a conservative form, for the general curvilinear coordinate
%system as
%%
%\begin{equation}
%	\frac{\partial \hat{Q}}{\partial t} + \frac{\partial \hat{E}}{\partial x} +
%	\frac{\partial \hat{F}}{\partial y} + \frac{\partial \hat{G}}{\partial z} = 0 \, \mbox{,}
%	\label{eq:vec-hat-RANS}
%\end{equation}
%%
%where 
%
%\begin{equation}
%	\hat{Q} = J^{-1}\overline{Q} = J^{-1} \left[ \overline{\rho} \quad \overline{\rho}\tilde{u} \quad 
%	\overline{\rho}\tilde{v} \quad \overline{\rho}\tilde{w} \quad \overline{e} \right]^{T} \quad \mbox{,}
%	\label{eq:hat_Q_vec}
%\end{equation}
%
%and the new flux vectors are given by
%%
%\begin{eqnarray}
%	\hat{E} = J^{-1} \left( 
%	\xi_{t}\overline{Q} + \xi_{x}\overline{E} + \xi_{y}\overline{F} + \xi_{z}\overline{G} 
%	\right) \, \mbox{,} \nonumber \\
%	\hat{F} = J^{-1} \left( 
%	\eta_{t}\overline{Q} + \eta_{x}\overline{E} + \eta_{y}\overline{F} + \eta_{z}\overline{G} 
%	\right) \, \mbox{,} \\  
%	\hat{G} = J^{-1} \left( 
%	\zeta_{t}\overline{Q} + \zeta_{x}\overline{E} + \zeta_{y}\overline{F} + \zeta_{z}\overline{G} 
%	\right) \, \mbox{.} \nonumber
%\end{eqnarray}
%
%Finally, the flux vectors are split in inviscid and viscous part in order to simplify the implementation. 
%Therefore, Eq.\ \eqref{eq:vec-hat-RANS} can be rewritten as
%%
%\begin{equation}
%	\frac{\partial \hat{Q}}{\partial t} + \frac{\partial \hat{E}_{e}}{\partial x} +
%	\frac{\partial \hat{F}_{e}}{\partial y} + \frac{\partial \hat{G}_{e}}{\partial z} = 
%	\frac{\partial \hat{E}_{v}}{\partial x} + \frac{\partial \hat{F}_{v}}{\partial y} + 
%	\frac{\partial \hat{G}_{v}}{\partial z} \, \mbox{,}
%	\label{eq:vec-hat-split-RANS}
%\end{equation}
%

The viscous flux vectors, $\hat{\mathbf{E}}_{v}$, $\hat{\mathbf{F}}_{v}$ and 
$\hat{\mathbf{G}}_{v}$, are written as
%
\begin{equation}
	\hat{\mathbf{E}}_{v} = J^{-1} \left\{\begin{array}{c}
		0 \\
		\xi_{x}\hat{\tau}_{xx} +  \xi_{y}\hat{\tau}_{xy} + \xi_{z}\hat{\tau}_{xz} \\
		\xi_{x}\hat{\tau}_{xy} +  \xi_{y}\hat{\tau}_{yy} + \xi_{z}\hat{\tau}_{yz} \\
		\xi_{x}\hat{\tau}_{xz} +  \xi_{y}\hat{\tau}_{yz} + \xi_{z}\hat{\tau}_{zz} \\
		\xi_{x}{\beta}_{x} +  \xi_{y}{\beta}_{y} + \xi_{z}{\beta}_{z} 
	\end{array}\right\} \, \mbox{,}
	\label{eq:hat-flux-Ev}
\end{equation}
%
\begin{equation}
	\hat{\mathbf{F}}_{v} = J^{-1} \left\{\begin{array}{c}
		0 \\
		\eta_{x}\hat{\tau}_{xx} +  \eta_{y}\hat{\tau}_{xy} + \eta_{z}\hat{\tau}_{xz} \\
		\eta_{x}\hat{\tau}_{xy} +  \eta_{y}\hat{\tau}_{yy} + \eta_{z}\hat{\tau}_{yz} \\
		\eta_{x}\hat{\tau}_{xz} +  \eta_{y}\hat{\tau}_{yz} + \eta_{z}\hat{\tau}_{zz} \\
		\eta_{x}{\beta}_{x} +  \eta_{y}{\beta}_{y} + \eta_{z}{\beta}_{z} 
	\end{array}\right\} \, \mbox{,}
	\label{eq:hat-flux-Fv}
\end{equation}
%
\begin{equation}
	\hat{\mathbf{G}}_{v} = J^{-1} \left\{\begin{array}{c}
		0 \\
		\zeta_{x}\hat{\tau}_{xx} +  \zeta_{y}\hat{\tau}_{xy} + \zeta_{z}\hat{\tau}_{xz} \\
		\zeta_{x}\hat{\tau}_{xy} +  \zeta_{y}\hat{\tau}_{yy} + \zeta_{z}\hat{\tau}_{yz} \\
		\zeta_{x}\hat{\tau}_{xz} +  \zeta_{y}\hat{\tau}_{yz} + \zeta_{z}\hat{\tau}_{zz} \\
		\zeta_{x}{\beta}_{x} +  \zeta_{y}{\beta}_{y} + \zeta_{z}{\beta}_{z} 
	\end{array}\right\} \, \mbox{,}
	\label{eq:hat-flux-Gv}
\end{equation}
%
where $\beta_{x}$, $\beta_{y}$ and $\beta_{z}$ are defined as
%
\begin{eqnarray}
	\beta_{x} = \hat{\tau}_{xx}\tilde{u} + \hat{\tau}_{xy}\tilde{v} +
	\hat{\tau}_{xz}\tilde{w} - \overline{q}_{x} \, \mbox{,} \nonumber \\
	\beta_{y} = \hat{\tau}_{xy}\tilde{u} + \hat{\tau}_{yy}\tilde{v} +
	\hat{\tau}_{yz}\tilde{w} - \overline{q}_{y} \, \mbox{,} \\
	\beta_{z} = \hat{\tau}_{xz}\tilde{u} + \hat{\tau}_{yz}\tilde{v} +
	\hat{\tau}_{zz}\tilde{w} - \overline{q}_{z} \mbox{.} \nonumber
\end{eqnarray}
%
and $\hat{\tau}_{ij}$ is given by
%
\begin{equation}
	\hat{\tau}_{ij} = 2 \left( \mu + \mu_{sgs}\right) 
	\left( \check{S}_{ij} - \frac{1}{3} \check{S}_{kk} \right) \, \mbox{.}
\end{equation}



==> sources/dimlss/dimlss.tex <==
\section{Dimensionless Formulation}

A convenient nondimensionalization is necessary in to order to achieve a consistent 
implementation of the governing equations of motion. Dimensionless formulation 
yields to a more general numerical tool. There is no need to change the formulation 
for each configuration intended to be simulated. Moreover, dimensionless formulation 
scales all the necessary properties to the same order of magnitude which is a 
computational advantage \cite{BIGA02}. Dimensionless variables are presented in the 
present section in order perform the nondimensionalization of Eq.\ 
\eqref{eq:vec-LES}

The dimensionless time, $\underline{\mathcal{T}}$, is written as function of the 
speed of sound of the jet at the inlet, $a_{j}$, and of a reference lenght, $l$,
%
\begin{equation}
	\underline{\mathcal{T}} = \mathcal{T} \frac{a_{j}}{l} \, \mbox{.}
	\label{eq:non-dim-time}
\end{equation}
%
In the present work $l$ represents the jet entrance diameter $d$. This reference lenght is 
also applied to write the dimensionless length, 
%
\begin{equation}
	\underline{l} = \frac{l}{d} \, \mbox{.}
	\label{eq:non-dim-lengh}
\end{equation}
%
The dimensionless velocity components are obtained using the speed of sound of the 
jet at the inlet,
%
\begin{equation}
	\underline{\textbf{u}} = \frac{\textbf{u}}{a_{j}} \, \mbox{.}
	\label{eq:non-dim-vel}
\end{equation}
%
Dimensionless pressure and energy are calculated using density and speed of the sound
of the jet at the inlet as
%
\begin{equation}
	\underline{p} = \frac{p}{\rho_{j}a_{j}^{2}} \, \mbox{,}
	\label{eq:non-dim-press}
\end{equation}
%
\begin{equation}
	\underline{E} = \frac{E}{\rho_{j}a_{j}^{2}} \, \mbox{.}
	\label{eq:non-dim-energy}
\end{equation}
%
Dimensionless density, $\underline{\rho}$, temperature, $\underline{T}$ and 
viscosity, $\underline{\mu}$, are calculated using freestream properties
%
\begin{equation}
	\underline{\rho} = \frac{\rho}{\rho_{j}} \, \mbox{.}
	\label{eq:non-dim-rho}
\end{equation}

One can use the dimensionless properties described above in order to write the 
dimensionless form of the RANS equations as
%
\begin{equation}
	\frac{\partial \underline{Q}}{\partial \mathcal{T}} + 
	\frac{\partial \underline{\mathbf{E}}_{e}}{\partial \xi} +
	\frac{\partial \underline{\mathbf{F}}_{e}}{\partial \eta} + 
	\frac{\partial \underline{\mathbf{G}}_{e}}{\partial \zeta} =
	\frac{1}{Re} \left( \frac{\partial \underline{\mathbf{E}}_{v}}{\partial \xi} 
	+ \frac{\partial \underline{\mathbf{F}}_{v}}{\partial \eta} 
	+ \frac{\partial \underline{\mathbf{G}}_{v}}{\partial \zeta} \right)	\, \mbox{,}
	\label{eq:vec-underline-split-RANS}
\end{equation}
%
where the underlined terms are calculated using dimensionless properties and the Reynolds number
is based on the jet properties such as the speed of sound, $a_{j}$, density, $\rho_{j}$, viscosity,
$\mu_{j}$ and the jet entrance diameter, $d$,
%
\begin{equation}
	Re = \frac{\rho_{j}a_{j}d}{\mu_{j}} \, \mbox{.}
\end{equation}



==> sources/introduction/introduction.tex <==
\section{Introduction}

One of the main design issues related to launch vehicles 
lies on noise emission originated from the complex 
interaction between the high-temperature/high-velocity 
exhaustion gases and the atmospheric air. These emissions 
yield very high noise levels, which must be minimized due
to several design constraints. For instance, the 
resulting pressure fluctuations can damage the solid 
structure of different parts of the launcher by 
vibrational acoustic stress. Therefore, it is a design
constraint to consider the loads resulting from acoustic 
sources in the structural dimensioning of large launch 
vehicles during the take 
off and also during the transonic flight. Moreover,
one cannot neglect the energy dissipation effect 
caused by the acoustic waves generated even if the 
vehicles is far from the ground. Theoretically, all 
chemical energy should be converted into kinectic
energy. However, in reallity, the noise generation 
consumes part of the chemical energy.

The acoustic design constraints have encouraged the 
studies of aeroacoustic fields around compressible jet 
flows. Instituto de Aeronautica e Espa\c{c}o (IAE) 
in Brazil is interested in this flow configuration for 
rocket design applications. Unsteady property fields of 
the flow are necessary for the aerocoustic studies. 
Therefore, the present work addresses the 
numerical study of unsteady turbulent compressible jet flows 
for such aeroacoustic applications. More precisely, on the
effects of subgrid scale modeling on 2nd order centered schemes
for compressible LES. A new computational tool is developed regarding 
the study of unsteady turbulent compressible flow. JAZzY is a novel 
large eddy simulation tool which is developed in order to reproduce 
high fidelity results of compressible jet flows which are used for 
aeroacoustic studies using the Ffowcs Williams and Hawkings approach
\cite{Wolf_doc}.
%
%Therefore, the present work addresses the development
%of a new numerical tool for the study of unsteady turbulent 
%compressible jet flows for aeroacoustic applications. 
%The novel code uses the large eddy simulation (LES) formulation 
%due to recent successful results of such approach for similar flow 
%configurations \cite{Bodony05i8, Garnier09}. The 
%solver is an upgrade of a finite difference Reynolds-averaged 
%Navier-Stokes (RANS) solver developed to study turbulent flows 
%for aerospace applications \cite{BIGA02}. Generally, LES calculations
%demand very dense grids. Hence, 
%high performance computing (HPC) is a requirement for such 
%simulations. Dynamic memory allocation and parallel 
%computation capabilities have been added to the legacy code 
%\cite{BIGA02}.

The System I formulation \cite{Vreman1995} is used here in 
order to model the filtered terms of the energy equation. 
The Smagorinsky \cite{Smagorinsky63} model is the chosen  model 
to calculate the components of the subgrid scale (SGS) tensor. 
The Eidson \cite{eidson85} hypothesis is the chosen model to 
calculate the subgrid scale terms of the filtered energy equation. 
For the sake of simplicity, only perfectly expanded jet configurations 
are studied in the current work. The LES tool is validated through 
a comparison of results with numerical 
\cite{Bodony05i8, Mendez10} and experimental 
\cite{Tanna77, bridges2008turbulence} data. Moreover, the 
computational performance of the solver is evaluated and discussed.


==> sources/nomenclature/nomenclature.tex <==
%\newpage

\section*{Nomenclature}

\begin{multicols}{2}

\subsection*{Abbreviations}

1-D: One dimensional\\
2-D: Two dimensional\\
3-D: Three dimensional\\
CFD: Computational fluid dynamics\\
CFL: Courant-Friedrichs-Lewys number \\
CGNS: CFD general notation system\\
EDQNM: Eddy-damped quasi-normal Markovian\\
IAE: Instituto de Aeron\'{a}utica e Espa\c{c}o\\
LES: Large eddy simulation\\
MPI: Message passing interface\\
SGS: Subgrid scale

\subsection*{English Characters}

$a$: Speed of sound\\
$B_{i}$: Subgrid terms of energy equation \\
$C_{p}$: Specific heat at constant pressure\\
$C_{s}$: Smagorinsky constant\\
$C_{v}$: Specific heat at constant volume\\
$D$: Inlet diameter\\
$\mathbf{d}$: Artificial dissipation term\\
$\mathcal{D}$: SGS viscous diffusion term\\
$E$: Total energy per mass unity\\
$\mathbf{E}_{e}$: Inviscid flux vector in the axial direction\\
$\mathbf{E}_{v}$: Viscous flux vector in the axial direction\\
$\mathbf{F}_{e}$: Inviscid flux vector in the radial direction\\
$\mathbf{F}_{v}$: Viscous flux vector in the radial direction\\
$\mathbf{G}_{e}$: Inviscid flux vector in the azimuthal direction\\
$\mathbf{G}_{v}$: Viscous flux vector in the azimuthal direction\\
$J$: Jacobian of the coordinate transformation\\
$l$: Reference lenght\\
$M$: Mach number\\
$p$: Static pressure\\
$Pr$: Prandtl number\\
$q$: Heat flux vector\\
$\mathcal{Q}_{j}$: Components of SGS temperature flux\\
$R$: Gas constant\\
$\mathbf{R}$: Riemman invariant\\
$Re$: Reynolds number\\
$RHS$: Right hand side of the equation\\
$S_{1}$: Sutherland constant\\
$S_{ij}$: Components of rate-of-strain tensor\\
$Sp_{N}$: Speedup for N processors\\
$t$: time\\
$T$: Temperature\\
$T_{N}$: CPU time using N processors\\
$T_{s}$: CPU time using single processor\\
$\textbf{u}$: Velocity vector\\
$u$: Components of the velocity vector in a Catesian coordinate system\\
$U$: Component of the contravariant velocity in the axial direction\\
$V$: Component of the contravariant velocity in the radial direction\\
$\vec{n}$ : Unity outward normal vector\\
$W$: Component of the contravariant velocity in the azimuthal direction\\
$\mathcal{W}$: Modified conservative properties of Turkel and Vatsa artificial dissipation\\
$\textbf{x}$: Spacial coordinates of a Cartesian coordinate system\\

\subsection*{Greek Characters}

$\alpha_{l}$: Runge-Kutta constants\\
$\beta_{j}$: Viscous terms of energy equation\\
$\gamma$: Specific heat ratio\\
$\Delta t$: Time-step\\
$\mathcal{E}$: SGS viscous dissipation \\
$\epsilon$: Turkel and Vatsa artificial dissipation terms \\
$\zeta$: Azimuthal direction\\
$\eta$: Radial direction\\
$\kappa$: Thermal conductivity\\
$\lambda$: Spectral radius-based scaling factor\\
$\lambda_{\zeta}$: Spectral radii in the $\zeta$ direction\\
$\lambda_{\eta}$: Spectral radii in the $\eta$ direction\\
$\lambda_{\xi}$: Spectral radii in the $\xi$ direction\\
$\mu$: Dynamic viscosity\\
$\nu$: Kinematicc viscosity\\
$\xi$: Axial direction\\
$\Pi_{dil}$: SGS pressure-diatation\\
$\rho$: Density\\
$\sigma_{ij}$: Components of the SGS tensor\\
$\tau_{ij}:$ Shear-stress tensor\\

\subsection*{Subscripts}

$j$: Relative to the jet \\ 
$\infty$: Relative to the freestream \\
$e$: Relative to interior domain \\
$f$: Relative to boundary face \\
$sgs$: subgrid property

%\subsection*{Superscripts}

\end{multicols}


==> sources/results-old/results.tex <==
\section{Preliminary Numerical Results}

%---------------------------------------------------------------%
The present section is devoted to a preliminary study of a supersonic 
perfectly expanded jet flow. Results are compared with analytical, 
numerical and experimental data from the literature 
\cite{Mendez10,bridges2008turbulence}. 
The first LES results using the Smagorinsky SGS turbulence closure 
\cite{Smagorinsky63} are discussed. The flow is characterized by an 
unheated perfectly expanded inlet jet with a Mach number of 
$1.4$ at the domain entrance. Therefore, the pressure ratio, 
$PR = P_{j}/P_\infty$, and the temperature ratio, $TR=T_{j}/T_\infty$, 
between the jet exit and the ambient freestream are equal to one, 
$PR = 1$ and $TR=1$. The time step used in the simulation is constant 
and equal to $2.5 \times 10^{-4}$ in dimensionless form. The Reynolds number 
of the jet is $Re = 1.57 \times 10^{6}$. The radial and longitudinal 
dimensions of the smallest cell of the computational domain are given by 
$(\Delta \underline{r})_{min}=0.002$ and $(\Delta \underline{x})_{min}=0.0126$, 
respectively, again in dimensionless form. This cell is located in the shear 
layer of the jet, at the entrance of the computational domain. The number 
of points in the azimuthal direction is $N_\theta=180$. The mesh domain is 
composed by 14.4 million points. The present mesh reproduces well the 
main geometric characteristics of the reference grid\cite{Mendez10}.

Data were extracted from the study after 35 dimensionless time
simulation, which represents approximately 4 flow-throught simulation for a 
1.4 dimensionless velocity. One flow through time is the time for a particle 
to cross the entire domain from the jet entrance to the domain exit.
The reader should remember that, as $TR=1$ and $a_j = a_\infty$, the  
characteristic time in the present work is equal to that reported in the work 
of Mendez \cite{Mendez10}. The preliminary simulation is performed in order to 
achieve a statiscaly stationary flow. After the preliminary study the simulation
is performed for more 40 dimensionless times, in which data were extracted 
each 0.02 dimensionless time in order to calculate time averaged properties.

Figure \ref{fig:lat-u-av} presents a lateral view of the time averaged axial component 
of velocity of the jet and Fig.\ \ref{fig:front-u-av} presents a frontal view of the 
jet at different positions in reference to the entry of the jet, in which $D$ represents 
the diameter of the jet at the inlet. Figure \ref{fig:profile-u-av} illustrates a comparison 
of profiles of averaged axial component of velocity at different postions to the inlet domain. 
The present results, blue line, are compared with the numerical simulation of Mendez 
{\it et al.} \cite{Mendez10}, dashed line, and the experimental data of Bridges and Wernet, 
square points \cite{bridges2008turbulence}. One can notice that the current simulation
correlates well with the references until $X=2.5D$. The current study has presented to be very 
dissipative as the jet get closer to the output domain. 
%
% Averaged axial component of velocity
%
\begin{figure}[h]
	\centering
    {\includegraphics[width=0.5\textwidth]{sources/results/pictures/surfaces/surfXZ/U-surf-xz}}
	\caption{Lateral view of the averaged axial component of velocity}
	\label{fig:lat-u-av}
\end{figure}
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny X=0.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/Uav/U-surf-x0-5D}}
  \subfigure[\tiny X=2.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/Uav/U-surf-x2-5D}}
  \subfigure[\tiny X=5.0D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/Uav/U-surf-x5-0D}}
  \subfigure[\tiny X=10D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/Uav/U-surf-x10-0D}}
	\caption{Frontal view of the averaged axial component of velocity at different positions}
	\label{fig:front-u-av}
\end{figure}
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny X=0.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/Uav_x2-5_prof}}
  \subfigure[\tiny X=2.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/Uav_x5-0_prof}}
  \subfigure[\tiny X=5.0D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/Uav_x10-0_prof}}
  \subfigure[\tiny X=10D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/Uav_x15-0_prof}}
	\caption{Profiles of averaged axial component of velocity along the X coordinate}
	\label{fig:profile-u-av}
\end{figure}

The lateral view and the frontal view of the RMS axial component of velocity are presented in
Figs.\ \ref{fig:lat-u-rms} and \ref{fig:front-u-rms}. The profiles of RMS axial component of 
velocity is illustrated in Fig.\ \ref{fig:profile-u-rms}. The RMS profiles correlates better to 
the reference than the axial component of velocity profiles. However, it also need ajustments
as the current results tend to differ from the reference as the jet approaches the exit domain and
fails to represent the peak of the profiles. The same observation can be performed for the profiles of 
RMS radial component of velocity and RMS azimuthal component velocity presented in Figs.\ 
\ref{fig:profile-v-rms} and \ref{fig:profile-w-rms}.
%
% RMS axial component of velocity
%
\begin{figure}[h]
	\centering
    {\includegraphics[width=0.5\textwidth]{sources/results/pictures/surfaces/surfXZ/urms-surf-xz}}
	\caption{Lateral view of the RMS axial component of velocity}
	\label{fig:lat-u-rms}
\end{figure}
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny X=0.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/urms/urms-surf-x0-5D}}
  \subfigure[\tiny X=2.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/urms/urms-surf-x2-5D}}
  \subfigure[\tiny X=5.0D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/urms/urms-surf-x5-0D}}
  \subfigure[\tiny X=10D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/urms/urms-surf-x10-0D}}
	\caption{Frontal view of the RMS axial component of velocity at different positions}
	\label{fig:front-u-rms}
\end{figure}
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny X=0.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/urms_x2-5_prof}}
  \subfigure[\tiny X=2.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/urms_x5-0_prof}}
  \subfigure[\tiny X=5.0D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/urms_x10-0_prof}}
  \subfigure[\tiny X=10D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/urms_x15-0_prof}}
	\caption{Profiles of RMS axial component of velocity along the X coordinate}
	\label{fig:profile-u-rms}
\end{figure}
%
% RMS radial component of velocity
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny X=0.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/vrms_x2-5_prof}}
  \subfigure[\tiny X=2.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/vrms_x5-0_prof}}
  \subfigure[\tiny X=5.0D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/vrms_x10-0_prof}}
  \subfigure[\tiny X=10D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/vrms_x15-0_prof}}
	\caption{Profiles of RMS radial component of velocity along the X coordinate}
	\label{fig:profile-v-rms}
\end{figure}
%
% RMS azimuthal component of velocity
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny X=0.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/wrms_x2-5_prof}}
  \subfigure[\tiny X=2.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/wrms_x5-0_prof}}
  \subfigure[\tiny X=5.0D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/wrms_x10-0_prof}}
  \subfigure[\tiny X=10D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/wrms_x15-0_prof}}
	\caption{Profiles of RMS azimuthal component of velocity along the X coordinate}
	\label{fig:profile-w-rms}
\end{figure}

A Reynolds shear stress component, $\overline{u'v'}$,  is also compared in the present abstract.
Figures \ref{fig:lat-uv} and \ref{fig:front-uv} presents the lateral view and the frontal view of 
$\overline{u'v'}$ respectively. Profiles of the Reynolds shear stress component are also compared with 
the literature at different positions in Fig.\ \ref{fig:profile-uv}. One can notice that the present
simulation can reproduce the correct shape of $\overline{u'v'}$ profiles. However, it fails to represent 
the the peak of $\overline{u'v'}$ in all the comparisons performed. 
%
% Reynolds shear stress component of velocity
%
\begin{figure}[h]
	\centering
    {\includegraphics[width=0.5\textwidth]{sources/results/pictures/surfaces/surfXZ/uv-surf-xz}}
	\caption{Lateral view of the Reynolds shear stress}
	\label{fig:lat-uv}
\end{figure}
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny X=0.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/uv/uv-surf-x0-5D}}
  \subfigure[\tiny X=2.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/uv/uv-surf-x2-5D}}
  \subfigure[\tiny X=5.0D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/uv/uv-surf-x5-0D}}
  \subfigure[\tiny X=10D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/surfaces/surfYZ/uv/uv-surf-x10-0D}}
	\caption{Frontal view of the Reynolds shear stress}
	\label{fig:front-uv}
\end{figure}
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny X=0.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/uv_x2-5_prof}}
  \subfigure[\tiny X=2.5D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/uv_x5-0_prof}}
  \subfigure[\tiny X=5.0D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/uv_x10-0_prof}}
  \subfigure[\tiny X=10D]
    {\includegraphics[width=0.24\textwidth]{sources/results/pictures/profile/uv_x15-0_prof}}
	\caption{Profiles of Reynolds shear stress along the X coordinate}
	\label{fig:profile-uv}
\end{figure}
%

The evolution of the averaged axial component of velocity and the evolution of the RMS axial 
component of velocity along the centerline and the lipline are illustrated in Figs.\ 
\ref{fig:u-av} and \ref{fig:u-rms} respectively. As discussed before, one can observe that
the simulation is over dissipative. The core of the jet is much smaller than the one of the 
refrences. The second order scheme used in the present simulation is very dissipative for 
coarse meshes, such as the the one used for this preliminary study. For the final version of 
the article the authors intend to use a 70M points grid and more sophisticated SGS closures 
such as the Vreman model \cite{Vreman1995,Vreman95} and the dynamic Smagorinsky model 
\cite{moin91}.
%
% Axial component of velocity at the centerline
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny Centerline]
    {\includegraphics[width=0.45\textwidth]{sources/results/pictures/profile/Uav_centerline}}
  \subfigure[\tiny Lipline]
    {\includegraphics[width=0.45\textwidth]{sources/results/pictures/profile/Uav_lipline}}
	\caption{Averaged axial component of velocity along the centerline and lipline}
	\label{fig:u-av}
\end{figure}
%
% Urms velocity at the centerline
%
\begin{figure}[h]
  \centering
  \subfigure[\tiny Centerline]
    {\includegraphics[width=0.45\textwidth]{sources/results/pictures/profile/urms_centerline}}
  \subfigure[\tiny Lipline]
    {\includegraphics[width=0.45\textwidth]{sources/results/pictures/profile/urms_lipline}}
	\caption{RMS axial component of velocity along the centerline and lipline}
	\label{fig:u-rms}
\end{figure}

\FloatBarrier



==> sources/results/results.tex <==
\section{Study of Supersonic Jet Flow}

%---------------------------------------------------------------%
Four numerical studies are performed in the present research in 
order to study the use of 2nd-order spatial discretization on large 
eddy simulations of a perfectly expanded jet flow configuration.
The effects of mesh refinement and SGS models are compared in the 
present work. Two different meshes are created for the refinement 
study. The three SGS models implemented in the code, classic 
Smagorinsky, dynamic Smagorinsky and Vreman, are compared in the 
current section. Results are compared with analytical, numerical 
and experimental data from the literature \cite{Mendez10,Mendez12,
bridges2008turbulence}. 

\subsection{Geometry Characteristics}

Two different geometries are created for the simulations discussed
in the current work. One geometry presents a cylindrical shape 
and the other one presents a divergent conical shape.
For the sake of simplicity, the round geometry is named geometry 
A and the other one is named geometry B in present text.
%
The computational domains are created in two steps. First, a 2-D 
region is generated. In the sequence, this region is rotated in 
order to generate a fully 3-D geometry. An in-house code is used 
for the generation of the 2-D domain of geometry A. The commercial 
mesh generator ANSYS\textsuperscript{\textregistered} ICEM CFD 
\cite{ICEM} is used for the 2-D domain of geometry B. 

%The 2-D regions are created using auxiliary zones in order to support 
%the mesh ge\-ne\-ra\-ti\-on. Figures \ref{fig:domain-a} and 
%\ref{fig:domain-b} present the mapping used for the creation of zones 
%of geometry A and geometry B, respectively. The zones are numerated 
%as indicated in the figures. The nozzle is not included into the 
%geometries used in the research. The domains are dimensionless in 
%order to be consistent with the mathematical approach used in JAZzY. 
%Therefore, a spatial unit represents one diameter of the jet inlet, 
%which is located at the inferior corner at the left of the domain, 
%more specifically at $x=0$, $-0.5D\leq y \leq 0.5D$ and 
%$-0,5D\leq z \leq 0.5D$.
%%
%\begin{figure}[ht]
%       \begin{center}
%		   \subfigure[2-D generation of geometry A.]{
%           \includegraphics[width=0.475\textwidth]
%		   {./sources/results/pictures/geometry/domain-a.png} 
%		   \label{fig:domain-a}
%		   }
%		   \subfigure[generation of geometry B.]{
%           \includegraphics[width=0.475\textwidth]
%		   {./sources/results/pictures/geometry/domain-b.png} 
%		   \label{fig:domain-b}
%		   }
%		   \caption{Zone mappings used for the generation of 
%		   the computational domains.}\label{fig:zones-geom}
%	   \end{center}
%\end{figure}

The geometry A is a cylindrical domain with radius of $20D$ and and length 
of $50D$. % The 2-D domain is divided in two zones by a line whose function 
%is given by,
%%
%\begin{equation}
%	y(x)=y_{0} + \frac{\mathcal{S}}{2}\left( \left(x-x_{0}\right) 
%	    + \left[\left(x-x_{0}\right)^{2}\right]^{\frac{1}{2}}
%		+ \epsilon^{2}\right) \, \mbox{,}
%	\label{eq:pope-distr}
%\end{equation}
%%
%where
%%
%\begin{eqnarray}
%	\displaystyle y_{0}=0.5D \, \mbox{,} & 
%	\displaystyle \mathcal{S}=0.094 \nonumber \, \mbox{,}\\
%	\displaystyle x_{0}=20.0D \, \mbox{,} & 
%	\displaystyle \epsilon=0.005 \, \mbox{.} \nonumber
%%	\label{eq:pope-const}
%\end{eqnarray}
%%
%Equation \eqref{eq:pope-distr} represents the jet spread according to 
%Pope \cite{Pope00}. The goal is to create a zone that supports a mesh 
%refinement which follows the growth of the jet along the longitudinal 
%direction. 
%
Geometry B presents a divergent form whose axis length is $40D$\@. The minimum 
and maximum heights of geometry B are $\approx 16D$ and $25D$, respectively.
The zones of this geometry are created based on results from simulations using
geometry A in order to refine the mesh in the shear layer region of the 
flow. % Table \ref{tab:zones-geom-b} provides the 2-D coordinates of the zones 
%created for geometry B. 
%%
%\begin{table}[htbp]
%\begin{center}
%\caption{Zone coordinates for geometry B}
%\label{tab:zones-geom-b}
%\begin{tabular}{|c|c|}
%\hline
%Zone Nb. & XY Coordinate \\
%\hline
%1 & $(0.00;0.00)$, $(0.00;15.00)$, $(15.01;0.15)$, $(0.00;0.25)$ \\
%\hline
%2 & $(15.00;0.00)$, $(25.00;0.00)$, $(25.00;0.15)$, $(15.01;0.15)$ \\
%\hline
%3 & $(25.00;0.00)$, $(40.00;0.00)$, $(40.00;0.15)$, $(25.00;0.15)$ \\
%\hline
%4 & $(00.00;0.25)$, $(15.01;0.15)$, $(14.93;1.54)$, $(00.00;0.50)$ \\
%\hline
%5 & $(15.01;0.15)$, $(25.00;0.15)$, $(25.00;2.25)$, $(14.93;1.54)$ \\
%\hline
%6 & $(25.00;0.15)$, $(40.00;0.15)$, $(40.00;3.30)$, $(25.00;2.25)$ \\
%\hline
%7 & $(0.00;0.50)$, $(14.93;1.54)$, $(14.70;3.31)$, $(-0.02;0.74)$ \\
%\hline
%8 & $(14.93;1.54)$, $(25.00;2.25)$, $(24.75;5.07)$, $(14.70;3.31)$ \\
%\hline
%9 & $(25.00;2.25)$, $(40.00;3.30)$, $(39.25;7.69)$, $(24.75;5.07)$ \\
%\hline
%10 & $(-0.02;0.74)$, $(14.70;3.31)$, $(13.56;11.27)$, $(-0.95;6.84)$ \\
%\hline
%11 & $(14.70;3.31)$, $(24.75;5.07)$, $(22.96;14.14)$, $(13.56;11.27)$ \\
%\hline
%12 & $(24.75;5.07)$, $(39.25;7.69)$, $(37.50;18.58)$, $(22.96;14.14)$ \\
%\hline
%13 & $(-0.95;6.84)$, $(13.56;11.27)$, $(12.34;16.06)$, $(-1.79;11.20)$ \\
%\hline
%14 & $(13.56;11.27)$, $(22.96;14.14)$, $(21.85;19.34)$, $(12.34;16.06)$ \\
%\hline
%15 & $(22.96;14.14)$, $(37.50;18.58)$, $(36.56;24.40)$, $(21.85;19.33)$ \\
%\hline
%\end{tabular}
%\end{center}
%\end{table}
%
Geometry A and geometry B are illustrated in Fig.\ \ref{fig:geom} which 
presents a 3-D view of the two computational domains used in the 
current work. The geometries are colored by a time solution of the axial 
component of velocity of the flow. 
%
%The computational domains are created in two steps. First, a 2-D region 
%is generated, as presented in Figs.\ \ref{fig:2d-geom-14m} and 
%\ref{fig:2d-geom-50m}. In the sequence, the 2-D domain is rotated in order 
%to generate the full 3-D domain, as illustrated in Figs.\ 
%\ref{fig:3d-geom-14m} and \ref{fig:3d-geom-50m}.   
%
\begin{figure}[htb!]
       \begin{center}
		   %\subfigure[2-D view of two XZ symatric plans of geometry A.]{
           %\includegraphics[width=0.475\textwidth]
		   %{./sources/results/pictures/geometry/2d-geom-14m.png} 
		   %\label{fig:2d-geom-14m}
		   %}
		   %\subfigure[2-D view of two XZ symatric plans of geometry B.]{
           %\includegraphics[width=0.475\textwidth]
		   %{./sources/results/pictures/geometry/2d-geom-50m.png} 
		   %\label{fig:2d-geom-50m}
		   %}
		   \subfigure[3-D view of two XZ plans of geometry A.]{
           \includegraphics[width=0.475\textwidth]
		   {./sources/results/pictures/geometry/3d-geom-14m.png} 
		   \label{fig:3d-geom-14m}
		   }
		   \subfigure[3-D view of two XZ plans of geometry B.]{
           \includegraphics[width=0.475\textwidth]
		   {./sources/results/pictures/geometry/3d-geom-50m.png} 
		   \label{fig:3d-geom-50m}
		   }
		   \caption{3-D view of geometries used for the LES.}
		   \label{fig:geom}
	   \end{center}
\end{figure}

\subsection{Mesh Configurations}

One grid is generated for each geometry used in the present study. These
computational grids are named mesh A and mesh B. The second mesh is created 
based on results using mesh A. One illustration of the computational 
grids is presented in Fig.\ \ref{fig:mesh-ab}. 
%
\begin{figure}[htb!]
       \begin{center}
		   \subfigure[2-D view of mesh A in the XZ plan.]{
           \includegraphics[width=0.475\textwidth]
		   {./sources/results/pictures/mesh/2d-mesh-14m.png} 
		   \label{fig:2d-mesh-14m}
		   }
		   %\subfigure[3-D view of mesh A in the XZ plan.]{
           %\includegraphics[width=0.475\textwidth]
		   %{./sources/results/pictures/mesh/3d-mesh-14m.png} 
		   %\label{fig:3d-mesh-14m}
		   %}
		   \subfigure[2-D view of mesh B in the XZ plan.]{
           \includegraphics[width=0.475\textwidth]
		   {./sources/results/pictures/mesh/2d-mesh-50m.png} 
		   \label{fig:2d-mesh-50m}
		   }
		   %\subfigure[3-D view of mesh B in the XZ plan.]{
           %\includegraphics[width=0.475\textwidth]
     	   %{./sources/results/pictures/mesh/3d-mesh-50m.png} 
		   %\label{fig:3d-mesh-50m}
		   %}
		   \caption{2-D view of the computational meshes 
		   used in the current work.}
		   \label{fig:mesh-ab}
	   \end{center}
\end{figure}
%
Mesh A is created using a mesh 
generator developed by the research group for the cylindrical shape 
configuration. This computational mesh is composed by 400 points in the axial 
direction, 200 points in the radial direction and 180 points in the azimuthal 
direction, which originates 14.4 million grid points. Hyperbolic tangent 
functions are used for the points distribution in the radial and axial 
directions. Grid points are clustered near the shear layer of the jet. The 
mesh is coarsened towards the outer regions of the domain in order to dissipate 
properties of the flow far from the jet. Such mesh refinement approach can avoid 
reflection of information into the domain. The radial and longitudinal dimensions 
of the smallest distance between mesh points of the computational grid are 
given by $(\Delta \underline{r})_{min}=0.002D$ and $(\Delta 
\underline{x})_{min}=0.0126D$, respectively. This minimal spacing occurs at the 
shear layer of the jet and at the entrance of the computational domain. Mesh A 
is created based on a reference grid of Mendez {\it et al.} \cite{Mendez10,
Mendez12}.

The refined computational grid is composed by 343 points in the axial 
direction, 398 points in the radial direction and 360 points in the 
azimuthal direction, which yields approximately 50 million grid 
points. The 2-D mesh is generated with ANSYS\textsuperscript{\textregistered} 
ICEM CFD \cite{ICEM}. The points are allocated using different 
distributions in eight edges of the 2-D domain. The same coarsening 
approach used for mesh A is also applied for mesh B. The distance 
between mesh points increase towards the outer region of the domain. 
This procedure force the dissipation of properties far from the jet 
in order to avoid reflection of data into the domain. The reader can 
find more details about the mesh generation on the work of Junqueira-Junior
\cite{Junior16}.

%Figure 
%\ref{fig:mesh-alloc} illustrate the edges used to generate 
%the points distribution and the direction of the mesh coarsening. 
%Table \ref{tab:mesh-b} presents the number of points, the growth 
%factor and the smallest grid spacing for all auxiliary edges 
%used to generate the mesh.
%%
%\begin{figure}[htb!]
%       \begin{center}
%           \includegraphics[width=0.5\textwidth]
%		   {./sources/results/pictures/mesh/strech.png} 
%		   \caption{Auxiliary edges of mesh used for geometry B.}
%		   \label{fig:mesh-alloc}
%	   \end{center}
%\end{figure}
%%
%\begin{table}[htbp]
%\begin{center}
%	\caption{Characteristics of mesh B}
%\label{tab:mesh-b}
%\begin{tabular}{|c|c|c|c|}
%\hline
%Edge & Nb. of points & Growth factor & Smallest spacing\\
%\hline
%a & 300 & 1.01912 & 0.100E-2D   \\
%b & 30  & 1.02739 & 28.231E-2D  \\
%c & 15  & 1.30370 & 34.4828E-2D \\
%d & 45  & 1.00    & ---------   \\
%e & 155 & 1.03724 & 0.340909E-2D\\
%f & 155 & 1.01034 & 1.18655E-2D \\
%g & 40  & 1.07161 & 5.73327E-2D \\
%h & 7   & 1.08206 & 79.3887E-2D \\
%\hline
%\end{tabular}
%\end{center}
%\end{table}

%\FloatBarrier

\subsection{Flow Configuration and Boundary Conditions}

An unheated perfectly expanded jet flow is chosen to validate the
LES tool. The flow is characterized by an unheated perfectly 
expanded inlet jet with a Mach number of $1.4$ at the domain 
entrance. Therefore, the pressure ratio, $PR=P_{j}/P_\infty$, 
and the temperature ratio, $TR=T_{j}/T_\infty$, between the jet 
exit and the ambient freestream conditions, are equal to one, {\em i.e.}, $PR = 1$ and $TR=1$. 
The Reynolds number of the jet is $Re=1.57 \times 10^{6}$, based on the jet exit diameter. This 
flow configuration is chosen due to the absence of strong shocks 
waves. Strong discontinuities must be carefully treated using 
numerical approaches which are not yet implemented into the 
solver. Moreover, numerical and experimental data of this flow
configuration are available in the literature such as the work 
of Mendez {\it et al.} \cite{Mendez10, Mendez12} and the work of 
Bridges and Wernet \cite{bridges2008turbulence}.

The boundary conditions discussed in section \ref{sec:BC} are used 
in the simulations performed in the current thesis. Figure 
\ref{fig:bc} presented a lateral view and a frontal view of the 
computational domain used by the simulation in where the positioning 
of each boundary condition is indicated. A flat-hat velocity profile, 
with $M=1.4$, is used at the entrance boundary. Riemann invariants are 
used at the farfield regions. A special singularity treatment is 
performed at the centerline. A periodicity is imposed in the azimuthal 
direction in order to create a transparency for the flow. 
%
%\begin{figure}[htb!]
%       \begin{center}
%		   \subfigure[Lateral view of boundary conditions.]{
%           \includegraphics[width=0.475\textwidth]
%		   {./sources/results/pictures/bc/bc-1.png} 
%		   \label{fig:bc-1}
%		   }
%		   \subfigure[Frontal view of boundary conditions.]{
%           \includegraphics[width=0.475\textwidth]
%		   {./sources/results/pictures/bc/bc-2.png} 
%		   \label{fig:bc-2}
%		   }
%		   \caption{Lateral and frontal views of the computational domain 
%		   indicating boundary conditions.}
%		   \label{fig:bc}
%	   \end{center}
%\end{figure}

Properties of flow at the inlet and at the farfield regions have to be 
provided to the code in order to impose the boundary conditions. Density, 
$\rho$, temperature, $T$, velocity, $U$, Reynolds number $Re$, and specific 
heat at constant volume, $C_{v}$, are provided in the dimensionless form 
to the simulation. These properties are given by
%
\begin{eqnarray}
	\rho_{j} = 1.00 \, \mbox{,} & 
	\rho_{\infty} = 1.00 \, \mbox{,} \nonumber \\
	T_{j} = 1.00 \, \mbox{,} & 
	T_{\infty} = 1.00 \, \mbox{,} \\
	U_{j} = 1.4 \, \mbox{,} & 
	U_{\infty} = 0.00 \nonumber \, \mbox{,}\\
	Re_{j}=1.57 \times 10^{6} \, \mbox{,}& 
	C_{v} = 1.786 \, \mbox{,} \nonumber
\end{eqnarray}
%
where the $j$ subscript stands for property at the jet entrance and the 
$\infty$ subscript stands for property at the farfield region. 

%\subsection{Reference Data}
%
%The present section is devoted to the presentation of technical
%details of the experimental data and numerical results used to 
%validade the simulations performed in the present work. The flow 
%conditions, numerical discretization, boundary and initial conditions
%of the references are discusses in the current section.
%
%The experimental data used to compared with LES simulations results 
%are obtained at the {\it Small Hot Jet Acoustic Ring} (SHJAR), located 
%within the AeroAcoustic Propulsion La\-bo\-ra\-to\-ry (AAPL) at NASA 
%Glenn Research center. Perfectly expanded flow results from the study 
%of Bridges and Wernet \cite{bridges2008turbulence}, using the SHJAR 
%apparatus, are used as an experimental reference in the present work. 
%
%A converging-diverging nozzle is used in the experiment. The Mach 
%number at the exit of the nozzle is 1.4\@. The nozzle exit diameter 
%is $D=50.8\mbox{mm}$ ($2.0$ inches). The lengh of the nozzle 
%is $7.55D$ and its initial diameter is $3D$. Therefore, the area of 
%contraction between the inlet and the outlet of the nozzle is 9:1. 
%The throat of the nozzle is located at $0.93D$ from the exit towards 
%the inlet section of the nozzle. The cross-section area at the throat 
%is $\approx 90\%$ of the exit area. The velocity of the jet measured 
%at the exit of the nozzle is $480.97\,[m/s]$ for $M=1.4$ and the 
%Reynolds of jet for the experiment, consedering the exit nozzle 
%diameter, is $\approx 1.57\times10^{6}$.
%
%The numerical data are extracted from the work of Mendez {\it et al.}
%\cite{Mendez10,Mendez12}. Numerical results of jet flows are achieved
%using a 2nd-order finite-volume scheme for 
%unstructured grids with the addition of 4th-order 
%stable artificial dissipation \cite{svard06}. Time integration is performed
%by an hybrid implicit-explicit scheme. 
%
%The nozzle is included into the geometry used by Mendez {\it et al}. 
%The mesh used on the simulation has 17 millions cells. 
%%This mesh is not refined in the wall regions of the nozzle. 
%A flat hat velocity profile is imposed at the nozzle inlet condition with 
%a hyperbolic tangent profile near the wall. The mesh used in the reference 
%is not sufficiently refined at the wall region which originates laminar 
%boundary layers at the exit of the nozzle. A very slow free-stream condition 
%(M=0.008) is used outside the nozzle. The thermodynamic characteristics of 
%this external flow correspond to the ambient conditions. A sponge treatment 
%is performed in order to avoid spurious reflection at the boundaries. The 
%numerical data is calculated using the dynamic Smagorinsky SGS model 
%\cite{moin91} and a Reynolds number of $Re=150,000$ which is smaller than 
%the one from the experimental data. The simulation is run four approximately 
%2 flow-throught times (FTT) in order to achieve a statiscally stateady state 
%before extracting data. In the sequence, more 4 FTT are performed in order to
%to calculate averaged properties and its fluctuations. One flow through time 
%is the time for a particle to cross the entire domain from the jet entrance to 
%the domain exit
%
%%\FloatBarrier
%
\subsection{Large Eddy Simulations}

Four simulations are performed in the present. The objective is to 
study the effects of mesh refinement and to evaluate the three 
different SGS models included into the code. The calculations are 
performed in two steps. First a preliminary simulation is performed 
in order to achieve a statistically steady state condition. In the 
sequence, the simulations are run for another period in order to 
collect enough data for the calculation of time averaged properties 
of the flow and its fluctuations. 

%\subsection{Statistically Steady Flow Condition} \label{sec:stat-steady-flow}

The configurations of all simulations are discussed in the current section,
towards the description of the preliminary calculations which are performed
in order to drive the flow to a statistically steady flow condition. Table 
\ref{tab:simu} presents the operating conditions of all four numerical 
studies performed in the current research. Mesh A is only used on S1. 
The other calculations are performed using the refined grid, Mesh B. The 
stagnated flow condition is used as initial condition for all simulations 
but S3, which uses the solution of S2 after 10.15 flow through times (FTT). 
One flow through time is the necessary time for a particle to cross all
the domain considering the inlet velocity of the jet. The dimensionless 
time increment used for all configurations is the biggest one which the 
solver can handle without diverging the solution. The static Smagorinsky
model \cite{Smagorinsky63,Lilly65,Lilly67} is used on S1 and S2. The
dynamic Smagorinsky model \cite{Germano91,moin91} and the Vreman model 
\cite{vreman2004} are used on S3 and S4, respectively.

The last column of Tab.\ \ref{tab:simu} represents the period simulated 
by all numerical studies in order to achieve the statistically steady state 
flow condition. The choice of this period is related to the computational 
cost of each study. S1 is the least expensive test case studied. It uses a 
14 million point mesh while the other simulations use the 50 million point grid. 
Therefore, S1 has been run for a longer period in order to achieve the statistically 
steady state condition. On the other hand, S3 is the most expensive numerical test 
case. The dynamic Smagorinsky SGS model, which is used by S3, needs more time per iteration 
when compared with the other SGS models implemented in the code. Hence, S3 has only been run 
for 5.86 FTT for this preliminary simulation. 
%
\begin{table}[htbp]
\begin{center}
	\caption{Configuration of large eddy simulations performed 
	in the present work}
\label{tab:simu}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Simulation & Mesh & SGS & $\Delta t$ & Initial condition & FTT \\
\hline
S1 & A & Static Smagorinsky  & $2.5 \times 10^{-5}$ & \small Stagnated flow & 37.8 \\
S2 & B & Static Smagorinsky  & $1 \times 10^{-4}$ & \small Stagnated flow  & 10.15 \\
S3 & B & Dynamic Smagorinsky & $5 \times 10^{-5}$ & \small Stagnated flow  & 5.86  \\
S4 & B & Vreman & $1 \times 10^{-4}$ & \small S2 -- 10.15 FTT & 13.65\\
\hline
\end{tabular}
\end{center}
\end{table}

%\subsection{Mean Flow Properties Calculation}

The simulations are restarted and run for another period in which 
data of the flow are extracted and recorded in a fixed frequency
after the preliminary study. The collected data are time averaged 
in order to calculate mean properties of the flow and compare with 
the results of the numerical and experimental references.


In the present work, time averaged properties are notated as 
$\langle \cdot \rangle$. Table \ref{tab:mean-simu} presents the 
configuration of simulations performed in order to calculate mean 
flow properties. The second column presents the number of extractions 
performed during the simulations. Data are extracted each 0.02 
dimensionless time in the present work which is equivalent to a 
dimensionless frequency of 50\@. The choice of this frequency is based 
on the numerical work reported in Refs.\ \citen{Mendez10} and \citen{Mendez12}. The last two 
columns of Tab.\ \ref{tab:mean-simu} present the total dimensionless 
time simulated to calculate the mean properties.
%
\begin{table}[htbp]
\begin{center}
	\caption{Time average configuration}
\label{tab:mean-simu}
\begin{tabular}{|c|c|c|c|}
\hline
Simulation & Nb. Extractions & Frequency & Total time \\
\hline
S1 & 2048 & 50 & 40.96 (1.14 FTT)\\
S2 & 3365 & 50 & 67.3  (2.36 FTT)\\
S3 & 2841 & 50 & 56.6  (1.98 FTT)\\
S4 & 1543 & 50 & 30.86 (1.08 FTT)\\
\hline
\end{tabular}
\end{center}
\end{table}

%In the present work time averaged properties, $\langle \cdot \rangle$,
%are calculated as
%%
%\begin{equation}
%	\langle x \rangle = \frac{1}{N} \sum_{i=1}^{N} x_{i}
%	\, \mbox{,}
%	\label{eq:mean}
%\end{equation}
%%
%where $N$ stands for the number of extractions. Root mean
%square (RMS) properties are calculated in order to probe the
%fluctiation part of properties. RMS properties as given by
%%
%\begin{equation}
%	x_{RMS} = \left[ \frac{1}{N} 
%	          \sum_{i=1}^{N} 
%			  \left(x_{i} - \langle x \rangle \right)^{2} 
%			  \right]^{\frac{1}{2}} \, \mbox{.}
%			  \label{eq:rms}
%\end{equation}
%%
%In the current research the components of the Reynolds stress 
%tensor are computed as
%%
%\begin{equation}
%	\langle x^{*} y^{*} \rangle = \frac{1}{N}
%	\sum_{i=1}^{N}\left[
%	\left( x_{i} - \langle x \rangle\right)
%	\left( y_{i} - \langle y \rangle\right)
%	\right]	\, \mbox{,}
%	\label{eq:mean-rey-comp}
%\end{equation}
%%
%in which the $*$ superscript stands for time fluctuation property.

%\subsection{Power Spectral Density Calculation}

A power spectral density (PSD) of the time fluctuation of the 
axial component of velocity, $u^{*}$, is calculated in order to 
study the transient part of the flow. The PSD computation is 
performed using the following methodology: first, sensors are 
included at three different positions along the lipline of the 
jet ($r/D=0.5$). For each position along the lipline, 120 sensors 
are allocated in the azimuthal direction. Information at this 
direction are averaged in order eliminate azimuthal dependence. 
Table \ref{tab:sensor} presents the positioning of the sensors 
in the axial and radial directions. The choice of the positioning 
is based on the numerical reference of Mendez {\it et. al.} 
\cite{Mendez10,Mendez12}. In the sequence, data are extracted 
from the sensors in order to generate a time-dependent signal.
The signal is partitioned into three equal parts and $u^{*}$ is 
calculated for all three partitioned signals. In the next step
of the methodology, the time fluctuation signals are multiplied 
by a window function in order to create periodic distribution. 
The Hamming window function \cite{harris1978} is used in the 
present work and it is written as
%
\begin{equation}
	w(n) = \alpha - \beta cos\left(\frac{2 \pi n}{N-1}\right)
	\, \mbox{,}
	\label{eq:window}
\end{equation}
%
where $\alpha=0.54$, $\beta=0.46$, $n$ stands for the time index 
and $N$ stands for the size of the sample. After applying the fast 
Fourier transformation (FFT) on the signals one can calculate the 
PSD of $u^{*}$. In the end, a simple average is applied on the three 
signals in order to have a final PSD of $u^{*}$ distribution.
%
\begin{table}[htbp]
\begin{center}
\caption{Positionig of the sensors used to collect fluctuation data}
\label{tab:sensor}
\begin{tabular}{|c|c|}
\hline
Signal & Positioning \\
\hline
(a) & $(X/D=0.10,r/D=0.5)$\\
(b) & $(X/D=0.25,r/D=0.5)$\\
(c) & $(X/D=1.25,r/D=0.5)$\\
\hline
\end{tabular}
\end{center}
\end{table}

In the present work the transient part is studied by the PSD of 
$u^{*}$ distribution as function of the number of Strouhal which 
is given by
%
\begin{equation}
	St(t) = \frac{\mathit{f}(t) D}{U_{j}} \, \mbox{,}
	\label{eq:strouhal}
\end{equation}
%
where $\mathit{f}$ stands for the frequency as a function of the time,
$D$ stands for the inlet diameter and $U_{j}$ stands for the velocity of
the jet at the entrance of the domain. Data are collected from the 
sensors using the same informations provided by Tab.\ \ref{tab:mean-simu}.
The minimum and maximum values of the Strouhal number for all simulations
are presented in Tab.\ \ref{tab:psd}.
%
\begin{table}[htbp]
\begin{center}
	\caption{Strouhal limits for all simulations}
\label{tab:psd}
\begin{tabular}{|c|c|c|}
\hline
Simulation & ${St}_{min}$ & ${St}_{max}$ \\
\hline
S1 & $1.74$ & 17.86\\
S2 & $1.06\times 10^{-2}$ & 17.86\\
S3 & $1.26\times 10^{-2}$ & 17.86\\
S4 & $2.31\times 10^{-2}$ & 17.86\\
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Study of Mesh Refinement Effects} \label{sec:mesh-study}

Effects of mesh refinement on compressible LES using the JAZzY 
solver are discussed in the present section. 2-D distribution
of properties and profiles of S1 and S2 are collected and 
compared with numerical and experimental results from the 
literature \cite{Mendez10,Mendez12,bridges2008turbulence}. 
Both simulations use the same SGS model, the static Smagorinsky
model \cite{Smagorinsky63,Lilly65,Lilly67}. Mesh A is used on S1 
and Mesh B is used on S2. Time averaged distributions of the axial 
component of velocity, density and eddy viscosity are presented in 
the subsection along with the RMS distribution of all three 
components of velocity, distributions of the $\langle u^{*}v^{*}
\rangle$ component of the Reynolds stress tensor and distributions
of the turbulent kinetic energy, $k$. Figure \ref{fig:extract} 
illustrates the positioning of surfaces and profiles extracted 
for all simulations performed in the current work.
%
\begin{figure}[htb!]
  \centering
    {\includegraphics[width=0.7\textwidth]
	{sources/results/pictures/extraction-14M}}
	\caption{Positioning in the computational domain of surfaces 
	studied in the present work}
	\label{fig:extract}
\end{figure}

\subsubsection*{Time Averaged Axial Component of Velocity}

One important characteristic of a round jet flow configurations is 
the potential core length, $\delta_{j}^{95\%}$. The potential 
core, $U_{j}^{95\%}$, is defined as $95\%$ of the velocity of 
the jet at the inlet,
%
\begin{equation}
	U_{j}^{95\%} = 0.95 \cdot U_{j}
	\, \mbox{.}
	\label{eq:pot-core}
\end{equation}
%
Therefore, the potential core length can be defined as the 
positioning in the centerline where $U_{j}^{95\%}$ is located.

Time averaged results of the axial component of velocity are 
presented in the subsection. A lateral view of $\langle U \rangle$ 
for S1 and S2, side by side, are presented in Fig.\ \ref{fig:lat-u-av-mesh}, 
where $U_{j}^{95\%}$ is indicated by the solid line. The positioning of surfaces is 
indicated in Fig.\ \ref{fig:extract}. Table \ref{tab:core-mesh} presents the size of 
the potential core of S1, S2 and the numerical results from Refs.\ \citen{Mendez10} 
and \citen{Mendez12}, along with the relative error compared with the experimental
data \cite{bridges2008turbulence}.
%
\begin{table}[htbp]
\begin{center}
  %\scalebox{0.5}{
  \caption{Potential core length and relative error of S1 and S2.}
  \label{tab:core-mesh}
  \begin{tabular}{|c|c|c|}
  \hline
  %Simulation & Potential core length $\delta_{j}^{95\%}$ & Relative error\\
  Simulation & $\delta_{j}^{95\%}$ & Relative error\\
  \hline
  S1 & 5.57 & 40\%\\
  S2 & 6.84 & 26\%\\
  Mendez {\it et al.} & 8.35 & 8\%\\
  \hline
  \end{tabular}
  %}
\end{center}
\end{table}
%
% Averaged axial component of velocity
%
\begin{figure}[htb!]
  \centering
%  \subfigure[$\langle U \rangle$ - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/XY/u-av-XY}}
%  \subfigure[$\langle U \rangle$ - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/XY/u-av-XY}}
  \subfigure[Lateral view of $\langle U \rangle$ for S1.]
    {\includegraphics[width=0.495\textwidth]
	{sources/results/pictures/stat-14m/XY-zoom/u-av-zoom-XY}}
  \subfigure[Lateral view of $\langle U \rangle$ for S2.]
    {\includegraphics[width=0.495\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/u-av-zoom-XY}}
	\caption{Lateral view of the averaged axial component of 
	velocity, $\langle U \rangle$, for S1 and S2. 
	(\LARGE \textbf{--}\scriptsize) indicates the 
	potential core of the jet, $U_{j}^{95\%}$.} 
	\label{fig:lat-u-av-mesh}
\end{figure}
%

Comparing the results, one can observe the difference in the 
potential core length between S1 and S2. The results of the 
first case present a smaller $\delta_{j}^{95\%}$ when compared to 
results of S2, {\em i.e.}, 5,57 and 6.84, respectively. One can say that 
the S1 solution is over dissipative when compared to the S2 
results. The jet vanishes earlier in S1\@. The mesh which is 
used in the S1 test case is very coarse when compared with the grid used 
for S2\@. This lack of resolution can generate very 
dissipative solutions which yield the under prediction of 
the potential core length. The mesh refinement reduced in 
14\% the relative error of S2 when compared to the 
experimental data. 

Profiles of $\langle U \rangle$ from S1 and S2, along the
mainstream direction, and the evolution of $\langle U \rangle$
along the centerline and along the lipline are compared 
with numerical and experimental results in Fig.\ \ref{fig:prof-u-av-mesh}. 
The centerline and the lipline are 
indicated as (E) and (F) in Fig.\ \ref{fig:extract}. The dash-point 
line and the solid line stand for the results of the S1 and S2 test cases,
respectively, in Fig.\ \ref{fig:prof-u-av-mesh}. The square symbols 
stand for the LES results of Mendez {\it et al.} \cite{Mendez10,
Mendez12}, while the triangular symbols stand for the experimental 
data of Bridges and Wernet \cite{bridges2008turbulence}.
%
\begin{figure}[htb!]
  \centering
  \subfigure[$\langle U \rangle$ - X=2.5D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/u-2-5-mesh}}
  \subfigure[$\langle U \rangle$ - X=5.0D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/u-5-0-mesh}}
  \subfigure[$\langle U \rangle$ - X=10D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/u-10-0-mesh}}
  \subfigure[$\langle U \rangle$ - X=15D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/u-15-0-mesh}}
  \subfigure[$\langle U \rangle$ - Centerline - Y=0 ; $0\leq X \leq 20D$ ]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/u-centerline-mesh}}
  \subfigure[$\langle U \rangle$ - Lipline - Y=0.5D ; $0\leq X \leq 20D$ ]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/u-lipline-mesh}}
	\caption{Profiles of averaged axial component of velocity at 
	different positions within the computational domain.
	(\LARGE \textbf{-}$\cdot$\textbf{-}\scriptsize), S1;
	(\LARGE \textbf{--}\scriptsize), S2; 
	($\square$), numerical data; ($\blacktriangle$), experimental data.}
	\label{fig:prof-u-av-mesh}
\end{figure}
%

The comparison of profiles indicates that distributions of 
$\langle U \rangle$ calculated on S1 and S2 correlates well 
with the references until $X=5.0D$. The $\langle U \rangle$ 
profile calculated with S2 at $X=10.0D$ is under predicted 
when compared with the reference profiles. However, it is 
closer to the reference when compared with the S1 results. 
One can notice that S1 and S2 $\langle U \rangle$ distributions 
along the centerline correlates with the references in the 
regions which the grid presents a good resolution. When the 
mesh spacing increases, due to the mesh coarsening in the 
streamwise direction, the time average axial component of 
velocity start to correlate poorly with the reference. The 
time averaged axial component of velocity calculated by S1, 
along the lipline, correlates better with the reference 
than the same property calculated on S2. The second case
overestimates the magnitude of $\langle U \rangle$ until 
$X\approx 6.0D$.

%\FloatBarrier

\subsubsection*{Root Mean Square Distribution of Time Fluctuations 
of Axial Velocity Component}

The time fluctuation part of the flow is also important to be studied.
The present work evaluates the axial and radial velocity components 
using the root mean square. A lateral view of $u^{*}_{RMS}$ computed 
by S1 and S2 simulations are presented in Figs.\ \ref{subfig:urms-det-s1}
and \ref{subfig:urms-det-s2}, respectively. The figures indicate that 
the property calculated by S1 is more spread when compared with the 
same property computed by S2. The mesh A refinement along with the 
spatial discretization can generate a more dissipative solution which 
creates the spread effect of $u^{*}_{RMS}$ calculated by S1 when compared
to the same property calculated by S2.
%
% RMS axial component of velocity
%
\begin{figure}[htb!]
  \centering
  \subfigure[Lateral view of $u^{*}_{RMS}$ for S1.]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/stat-14m/XY-zoom/u-rms-zoom-XY}\label{subfig:urms-det-s1}}
  \subfigure[Lateral view of $u^{*}_{RMS}$ for S2.]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/u-rms-zoom-XY}\label{subfig:urms-det-s2}}
  \subfigure[Lateral view of $v^{*}_{RMS}$ for S1.]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/stat-14m/XY-zoom/v-rms-zoom-XY}\label{subfig:vrms-det-s1}}
  \subfigure[Lateral view of $v^{*}_{RMS}$ for S2.]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/v-rms-zoom-XY}\label{subfig:vrms-det-s2}}
  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S1.]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/stat-14m/XY-zoom/uv-av-zoom-XY}\label{subfig:uv-det-s1}}
  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S2.]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/uv-av-zoom-XY}\label{subfig:uv-det-s2}}
	\caption{Lateral view of RMS of time fluctuation
	of axial component of velocity, $u_{RMS}^{*}$, RMS 
	of time fluctuation of radial component of velocity, 
	$v_{RMS}^{*}$ and $\langle u^{*}v^{*}\rangle$ Reynolds 
	shear stress tensor component, for S1 and S2.} 
	\label{fig:lat-u-v-uv-mesh}
\end{figure}
%

The same strategy used to compare the mean profiles of velocity is 
used here for the study of $u^{*}_{RMS}$. Figure \ref{fig:prof-u-rms-mesh}
presents the comparison of root mean square profiles of $u^{*}$
calculated by S1 and S2 with reference results. The profile of 
$u^{*}_{RMS}$ calculated by S2 fits perfectly the reference profiles 
at $X=2.5D$. The profile calculated by S1, at the same position, 
presents a good correlation with numerical and experimental data. 
However, it does not correctly represent the two peaks of the profile. 
For $X=5.0D$ and $X=10.0D$ the profiles start to diverge from the 
reference results. At $X=15.0D$, the $u^{*}_{RMS}$ profile, calculated 
by S1, present a different shape and different magnitude from the
reference profiles. At the same position the fluctuation profile 
computed by S2 reproduce the same peaks of the reference data. However, 
the shape of the profile is completely different from the shape of
profiles calculated by the references.
%
\begin{figure}[htb!]
  \centering
  \subfigure[$u^{*}_{RMS}$ - X=2.5D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/urms-2-5-mesh}}
  \subfigure[$u^{*}_{RMS}$ - X=5.0D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/urms-5-0-mesh}}
  \subfigure[$u^{*}_{RMS}$ - X=10D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/urms-10-0-mesh}}
  \subfigure[$u^{*}_{RMS}$ - X=15D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/urms-15-0-mesh}}
  \subfigure[$u^{*}_{RMS}$ - Centerline - Y=0 ; $0\leq X \leq 20D$ ]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/urms-centerline-mesh}\label{subfig:urms-centerline}}
  \subfigure[$u^{*}_{RMS}$ - Lipline - Y=0.5D ; $0\leq X \leq 20D$ ]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/urms-lipline-mesh}\label{subfig:urms-lipline}}
	\caption{Profiles of RMS of time fluctuation of axial 
	component of velocity, $u_{RMS}^{*}$, for S1 and S2,
	at different positions within the computational domain.
	(\LARGE \textbf{-}$\cdot$\textbf{-}\scriptsize), S1;
	(\LARGE \textbf{--}\scriptsize), S2; 
	($\square$), numerical data; ($\blacktriangle$), experimental data.}
	\label{fig:prof-u-rms-mesh}
\end{figure}
%

\FloatBarrier

Figures \ref{subfig:urms-centerline} and \ref{subfig:urms-lipline}
presents the distribution of $u^{*}_{RMS}$ along the centerline and 
lipline of the jet. The distributions calculated by S1 and S2 are
somewhat different from the results of the references. However,
one can notice an upgrade on the solution when comparing S1 and S2
results. The results achieved using the more refined mesh are closer
to the reference than the results obtained using mesh A.

\subsubsection*{Root Mean Square Distribution of Time Fluctuations 
of Radial Velocity Component}

The time fluctuation of the radial component of velocity is also 
compared with the reference data. Distributions of root mean square 
of $v_{RMS}^{*}$ are presented in the subsection. Figures 
\ref{subfig:vrms-det-s1} and \ref{subfig:vrms-det-s2} illustrate
a lateral view of the distribution of $v_{RMS}^{*}$ computed by S1 and S2,
respectively. A significant divergence between the results can be easily
noticed on the lateral view of the $v_{RMS}^{*}$ distribution. 
From $X=2.5D$ towards the exit boundary the magnitude of fluctuation 
calculated by S1 is much higher than the magnitude of $v_{RMS}^{*}$ 
computed by S2.

Four profiles of $v_{RMS}^{*}$ in the radial direction at $X=2.5D$, 
$X=5.0D$, $X=10.0D$ and $X=15.0D$ are presented in 
Fig.\ \ref{fig:prof-v-rms-mesh}. S1 results presented a good correlation 
with the reference at $X=2.5D$, where only the peaks of the profile 
are not well represented. For all other positions on the axial 
direction studied in the present research the $v_{rms}^{*}$
profiles of S1 are overestimated and poorly correlates with the 
reference. On the other hand, $v_{RMS}^{*}$ profiles calculated 
using a refined grid fits very well with the results of the numerical 
reference at $X=2.5D$ and $X=5.0D$. At $X=10.0D$ the fluctuation 
profile calculated by S2 presents a better correlation with the 
experimental data than the numerical reference. At $X=15.0D$ the S2
does not present a good profile of $v_{RMS}^{*}$.
%
%
% RMS radial component of velocity
%
%\begin{figure}[htb!]
%  \centering
%  %\subfigure[$v^{*}_{RMS}$ - S1]
%  %  {\includegraphics[width=0.495\textwidth]
%  %  {sources/results/pictures/stat-14m/XY/v-rms-XY}}
%  %\subfigure[$v^{*}_{RMS}$ - S2]
%  %  {\includegraphics[width=0.495\textwidth]
%  %  {sources/results/pictures/stat-cs/XY/v-rms-XY}}
%  \subfigure[Lateral view of $v^{*}_{RMS}$ for S1.]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/XY-zoom/v-rms-zoom-XY}}
%  \subfigure[Lateral view of $v^{*}_{RMS}$ for S2.]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/XY-zoom/v-rms-zoom-XY}}
%	\caption{Lateral view of RMS of time fluctuation
%	of radial component of velocity, $v_{RMS}^{*}$, for S1
%	and S2.} 
%	\label{fig:lat-v-rms-mesh}
%\end{figure}
%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$v^{*}_{RMS}$ - X=0.5D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-0-5/v-rms-0-5-YZ}}
%  \subfigure[$v^{*}_{RMS}$ - X=0.5D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-0-5-mesh/v-rms-0-5-YZ}}
%  \subfigure[$v^{*}_{RMS}$ - X=2.5D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-2-5/v-rms-2-5-YZ}}
%  \subfigure[$v^{*}_{RMS}$ - X=2.5D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-2-5-mesh/v-rms-2-5-YZ}}
%  \subfigure[$v^{*}_{RMS}$ - X=5.0D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-5-0/v-rms-5-0-YZ}}
%  \subfigure[$v^{*}_{RMS}$ - X=5.0D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-5-0-mesh/v-rms-5-0-YZ}}
%	\caption{Frontal views of RMS of time fluctuation
%	of radial component of velocity, $v_{RMS}^{*}$, for S1 and S2, 
%	at different positions along the axial coordinate. (\LARGE 
%	\textbf{-} \textbf{-}\normalsize) indicates the potential core 
%	of the jet, $U_{j}^{95\%}$.}
%	\label{fig:front-v-rms-mesh}
%\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure[$v^{*}_{RMS}$ - X=2.5D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/vrms-2-5-mesh}}
  \subfigure[$v^{*}_{RMS}$ - X=5.0D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/vrms-5-0-mesh}}
  \subfigure[$v^{*}_{RMS}$ - X=10D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/vrms-10-0-mesh}}
  \subfigure[$v^{*}_{RMS}$ - X=15D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/vrms-15-0-mesh}}
	\caption{Profiles of RMS of time fluctuation of radial 
	component of velocity, $v_{RMS}^{*}$, for S1 nd S2,
	at different positions within the computational domain.
	(\LARGE \textbf{-}$\cdot$\textbf{-}\scriptsize), S1;
	(\LARGE \textbf{--}\scriptsize), S2; 
	($\square$), numerical data; ($\triangle$), experimental data.}
	\label{fig:prof-v-rms-mesh}
\end{figure}

\subsubsection*{Component of Reynolds Stress tensor}

Figures \ref{subfig:uv-det-s1}, \ref{subfig:uv-det-s2} and 
\ref{fig:prof-uv-av-mesh} present lateral views and profiles of 
$\langle u^{*}v^{*}\rangle$ component of the Reynolds stress tensor.
One can observe that the distributions of the property obtained by S1 
is over dissipated when compared with results collected from S2. Comparing 
the profiles with the reference, one can notice that the profiles achived in 
S1 and S2 are really far from the numerical and ex\-pe\-ri\-men\-tal data. 
The solver has produced with succes the shape of $\langle u^{*}v^{*}\rangle$ 
profile. However, it fails to represent the peak of 
$\langle u^{*}v^{*}\rangle$ for all profiles compared.
%
% Reynolds shear stress component of velocity
%
%\begin{figure}[htb!]
%  \centering
%  %\subfigure[$\langle u^{*}v^{*}\rangle$ - S1]
%  %  {\includegraphics[width=0.415\textwidth]
%  %  {sources/results/pictures/stat-14m/XY/uv-av-XY}}
%  %\subfigure[$\langle u^{*}v^{*}\rangle$ - S2]
%  %  {\includegraphics[width=0.415\textwidth]
%  %  {sources/results/pictures/stat-cs/XY/uv-av-XY}}
%  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S1.]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/XY-zoom/uv-av-zoom-XY}}
%  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S2.]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/XY-zoom/uv-av-zoom-XY}}
%	\caption{Lateral view of the $\langle u^{*}v^{*}\rangle$ 
%	Reynolds shear stress tensor component, for S1 and S2.} 
%	\label{fig:lat-uv-av-mesh}
%\end{figure}
%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=0.5D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-0-5/uv-av-0-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=0.5D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-0-5-mesh/uv-av-0-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=2.5D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-2-5/uv-av-2-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=2.5D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-2-5-mesh/uv-av-2-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=5.0D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-5-0/uv-av-5-0-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=5.0D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-5-0-mesh/uv-av-5-0-YZ}}
%	\caption{Frontal views of the $\langle u^{*}v^{*} \rangle$
%	Reynolds shear stress tensor component for S1 and S2, 
%	at different positions along the axial coordinate. (\LARGE 
%	\textbf{-} \textbf{-}\normalsize) indicates the potential core 
%	of the jet, $U_{j}^{95\%}$.}
%	\label{fig:front-uv-av-mesh}
%\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=2.5D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/uv-2-5-mesh}}
  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=5.0D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/uv-5-0-mesh}}
  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=10D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/uv-10-0-mesh}}
  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=15D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/mesh/uv-15-0-mesh}}
	\caption{Profiles of the $\langle u^{*}v^{*} \rangle$ 
	Reynolds shear stress tensor component, for S1 and S2, at 
    different positions within the computational domain.
	(\LARGE \textbf{-}$\cdot$\textbf{-}\scriptsize), S1;
    (\LARGE \textbf{--}\scriptsize), S2;
    ($\square$), numerical data; ($\triangle$), experimental data.}
	\label{fig:prof-uv-av-mesh}
\end{figure}

\subsubsection*{Time Averaged Eddy Viscosity}

The effects of the mesh on the SGS modeling are also studied in 
the present subsection. Figure \ref{fig:lat-mut-mesh}
presents distributions of time averaged eddy viscosity, 
$\langle\mu_{t}\rangle$, calculated on S1 and S2. The Smagorinsky 
model \cite{Smagorinsky63,Lilly65,Lilly67} is used on both simulations. 
This SGS closure is highly dependent on the local mesh size. One can 
notice that $\langle\mu_{t}\rangle$ presents higher values on the 
distributions obtained by S1. On the other hand, the eddy viscosity is only 
acting on the regions where the mesh is no longer very refined for the 
S2 study. The $\langle\mu_{t}\rangle$ is very low in the region where 
the grid spacing is small.
%
% Turbulent viscosity
%
\begin{figure}[htb!]
  \centering
  %\subfigure[$\langle\mu_{t}\rangle$ - S1]
  %  {\includegraphics[width=0.495\textwidth]
  %  {sources/results/pictures/stat-14m/XY/mut-av-XY}}
  %\subfigure[$\langle\mu_{t}\rangle$ - S2]
  %  {\includegraphics[width=0.495\textwidth]
  %  {sources/results/pictures/stat-cs/XY/mut-av-XY}}
  \subfigure[Lateral view of $\langle\mu_{t}\rangle$ for S1.]
    {\includegraphics[width=0.495\textwidth]
	{sources/results/pictures/stat-14m/XY-zoom/mut-av-zoom-XY}}
  \subfigure[Lateral view of $\langle\mu_{t}\rangle$ for S2.]
    {\includegraphics[width=0.495\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/mut-av-zoom-XY}}
	\caption{Lateral view and detailed view of time averaged
	eddy viscosity, $\langle\mu_{t}\rangle$, for S1 and S2.} 
	\label{fig:lat-mut-mesh}
\end{figure}
%

The eddy viscosity can contribute to the dissipative 
characteristic of the simulations. Specially for meshes with
low point resolution. The divergence observed on the 
distribution of $\langle\mu_{t}\rangle$ calculated by S1 and S2
is an example of such effect. However, it is important to 
notice that, even in regions where the mesh is not very refined, 
yet, not coarse, and where the eddy viscosity can be neglected, 
some distributions of properties, calculated by S2, have shown to 
be very dissipative when compared with the LES reference and with
the experimental data. Therefore, one can state that the 
truncation errors originated from the second order spatial 
discretization, used on the simulations here performed, can easily 
overcome the effects of SGS modeling if the grid spacing is not 
small enough. The issue is very important for the structured mesh
approach. Increasing mesh resolution in the region of interest
expressively rises up the number of points all over the computational
domain. Local refinement for structured mesh is not straight 
forward and the code used in the current work does not have such 
approach available.

%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$\langle\mu_{t}\rangle$ - X=0.5D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-0-5/mut-av-0-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=0.5D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-0-5-mesh/mut-av-0-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=2.5D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-2-5/mut-av-2-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=2.5D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-2-5-mesh/mut-av-2-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=5.0D - S1]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-14m/YZ-5-0/mut-av-5-0-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=5.0D - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/YZ-5-0-mesh/mut-av-5-0-YZ}}
%	\caption{Frontal views of the time averaged eddy viscosity,
%	$\langle\mu_{t}\rangle$, for S1 and S2, at different positions along 
%	the axial coordinate. (\LARGE \textbf{-} \textbf{-}\normalsize) 
%	indicates the potential core of the jet, $U_{j}^{95\%}$.}
%	\label{fig:front-mut-mesh}
%\end{figure}

%\FloatBarrier

\subsubsection*{Power Spectral Density}

The power spectral density of time fluctuation of the axial component 
of velocity is studied in the present work in order to better 
understand the transient portion of the solution. Figure 
\ref{fig:psd-mesh} presents the PSD of $u^{*}$, in $dB$, as function 
of the Strouhal number for S1 and S2. The signals are collected from 
the sensors allocated at the positions presented in Tab.\ 
\ref{tab:sensor}. The PSD of $u^{*}$ are shifted of -150{\bf dB} 
and -300{\bf dB} for $X=0.25D$ and $X=1.25$, respectively, in order 
to separate plots. 

One can observe that PSD signals obtained using S1 and S2 present a 
similar behavior at $X=1.25D$ on the lipline. On the other hand, it 
is possible to notice significant differences on the shape and on the 
peaks positioning for $St>1.0$ at $X=0.1D$ and $X=0.25D$. The divergence 
indicates that the dissipative characteristic of S1 have changed the
positioning of the turbulent transition when compared with the S2 study.

\begin{figure}[htb!]
  \centering
    {\includegraphics[width=0.7\textwidth]
	{sources/results/pictures/comparison/psd/psd-lipline-mesh}}
	\caption{Power spectral density of $u^{*}$ as function of the Strouhal
	number along the lipline of the jet. 
	(\LARGE {\color{green}\textbf{--}}\scriptsize), S1; 
	(\LARGE \textbf{--}\scriptsize), S2. A shift of -150 {\bf dB} and 
	-300 {\bf dB} has been added to the PSD in order to separate plots 
	for $X=0.25D$ and $X=1.25D$, respectively.}
	\label{fig:psd-mesh}
\end{figure}

%\FloatBarrier

\subsection{Subgrid Scale Modeling Study}

After the mesh refinement study the three SGS models added
to the solver are compared. S2, S3 and S4 simulations
are performed using the static Smagorinsky model 
\cite{Smagorinsky63,Lilly65,Lilly67}, the dynamic Smagorinsky 
model \cite{germano90,moin91} and the Vreman model 
\cite{vreman2004}, respectively. The same mesh with 50 
million points is used for all three simulations.
The stagnated flow condition is used as intial condition
for S2 and S3. A restart of S2 is used as initial condition
for the S4 simulation. The configuration of the numerical 
studies is presented at Tab.\ \ref{tab:simu}. The same comparisons 
performed on the study of mesh refinement effects, Sec.\ 
\ref{sec:mesh-study}, are performed for the SGS modeling study.

\subsubsection*{Time Averaged Axial Component of Velocity}

Effects of the SGS modeling on the time averaged results of the 
axial component of velocity are presented in the subsection. A 
lateral view of $\langle U \rangle$ for S2, S3 and S4, side by 
side, are presented in Fig.\ \ref{fig:lat-u-av-sgs}, where 
$U_{j}^{95\%}$ is indicated by the solid line. 
%
\begin{figure}[htb!]
  \centering
  \subfigure[Lateral view of $\langle U \rangle$ for S2.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/u-av-zoom-XY}}
  \subfigure[Lateral view of $\langle U \rangle$ for S3.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-ds/XY-zoom/u-av-zoom-XY}}
  \subfigure[Lateral view of $\langle U \rangle$ for S4.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-vr/XY-zoom/u-av-zoom-XY}}
	\caption{Lateral view of the averaged axial component 
	of velocity, $\langle U \rangle$, for S2, S3 and S4.
	(\LARGE \textbf{--}\scriptsize) indicates the 
	potential core of the jet, $U_{j}^{95\%}$.} 
	\label{fig:lat-u-av-sgs}
\end{figure}
%
%Frontal views of $\langle U \rangle$ at three different surfaces, 
%calculated by the three simulations studied in the present section 
%are presented in Fig.\ \ref{fig:front-u-av-sgs}. 
%The positioning of surfaces is indicated in Fig.\ \ref{fig:extract}. 
%The dashed line in Fig.\ \ref{fig:front-u-av-sgs} represents the 
%potential core of the jet. 
Table \ref{tab:core-sgs} presents the size of 
the potetial core of S2, S3 and S4 and the numerical reference 
\cite{Mendez10,Mendez12} along with the relative error compared 
with the experimental data \cite{bridges2008turbulence}.
%
\begin{table}[htb!]
\begin{center}
  %\scalebox{0.5}{
  \caption{Potential core length and relative error of S2, S3 and S4.}
  \label{tab:core-sgs}
  \begin{tabular}{|c|c|c|}
  \hline
  %Simulation & Potential core length $\delta_{j}^{95\%}$ & Relative error\\
  Simulation & $\delta_{j}^{95\%}$ & Relative error\\
  \hline
  S2 & 6.84 & 26\%\\
  S3 & 6.84 & 26\%\\
  S4 & 6.28 & 32\%\\
  Mendez {\it et al.} & 8.35 & 8\%\\
  \hline
  \end{tabular}
  %}
\end{center}
\end{table}

Comparing the results, one cannot observe significant differences 
on the potential core length between S2, S3 and S4. The distribution
of $\langle U \rangle$ calculated using the dynamic Smagorinky model
has shown to be slightly more concentrated at the centerline region.
S2 and S4 time averaged distribution of $U$ are, on some small scale,
more spread than the distribution obtained by S3.

Profiles of $\langle U \rangle$ from S2, S3 and S4, along the
mainstream direction, and the evolution of $\langle U \rangle$
along the centerline and, also along the lipline, are compared 
with numerical and experimental results in Fig.\ \ref{fig:prof-u-av-sgs}.  
The solid line, the dashed line and 
the circular symbol stand for the profiles of $\langle U \rangle$
computed by S2, S3 and S4, respectively. The reference data are 
represented by the same symbols presented in the mesh refinement
study. 
%
\begin{figure}[htb!]
  \centering
  \subfigure[$\langle U \rangle$ - X=2.5D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/u-2-5-sgs}}
  \subfigure[$\langle U \rangle$ - X=5.0D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/u-5-0-sgs}}
  \subfigure[$\langle U \rangle$ - X=10D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/u-10-0-sgs}}
  \subfigure[$\langle U \rangle$ - X=15D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/u-15-0-sgs}}
  \subfigure[$\langle U \rangle$ - Centerline - Y=0 ; $0\leq X \leq 20D$ ]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/u-centerline-sgs}}
  \subfigure[$\langle U \rangle$ - Lipline - Y=0.5D ; $0\leq X \leq 20D$ ]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/u-lipline-sgs}}
	\caption{Profiles of averaged axial component of velocity at 
	different positions within the computational domain.
	(\LARGE \textbf{--}\scriptsize), S2; 
	(\LARGE \textbf{-}\textbf{-}\scriptsize), S3;
	($\bigcirc$), S4; ($\square$), numerical data; 
	($\blacktriangle$), experimental data.}
	\label{fig:prof-u-av-sgs}
\end{figure}
%


The comparison of profiles indicates that distributions of 
$\langle U \rangle$ calculated on S2, S3 and S4 correlates 
well with the references until $X=5.0D$. For $X>10.0D$ 
all SGS models fail to predict the correct profile.
One can notice that the evolution of $\langle U\rangle$
along the centerline, calculated by all three simulations,
are in good agreement with the numerical and experimental 
reference data at the region where the mesh presents a good 
resolution. Moreover, the three distributions calculated using
different SGS closures have presented the very similar behavior.
%
The dynamic Smagorinsky model and the Vreman model correlates
better with the experimental data for $X<5.0D$ than the classic 
Smagorinsky closure does. However, all simulations tend to not 
predict well the magnitude of $\langle U \rangle$ on the lipline
when the mesh size increases, $X>5.0D$. 

%\FloatBarrier

%\FloatBarrier

\subsubsection*{Root Mean Square Distribution of Time Fluctuations 
of Axial Velocity Component}

A lateral view of $u^{*}_{RMS}$ computed by S2, S3 and S4 simulations 
are presented in Figs.\ \ref{subfig:urms-sgs-s2}, \ref{subfig:urms-sgs-s3}
and \ref{subfig:urms-sgs-s4}, respectively. 
%
\begin{figure}[htb!]
  \centering
  \subfigure[Lateral view of $u^{*}_{RMS}$ for S2.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/u-rms-zoom-XY}\label{subfig:urms-sgs-s2}}
  \subfigure[Lateral view of $u^{*}_{RMS}$ for S3.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-ds/XY-zoom/u-rms-zoom-XY}\label{subfig:urms-sgs-s3}}
  \subfigure[Lateral view of $u^{*}_{RMS}$ for S4.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-vr/XY-zoom/u-rms-zoom-XY}\label{subfig:urms-sgs-s4}}
  \subfigure[Lateral view of $v^{*}_{RMS}$ for S2.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/v-rms-zoom-XY}\label{subfig:vrms-sgs-s2}}
  \subfigure[Lateral view of $v^{*}_{RMS}$ for S3.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-ds/XY-zoom/v-rms-zoom-XY}\label{subfig:vrms-sgs-s3}}
  \subfigure[Lateral view of $v^{*}_{RMS}$ for S4.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-vr/XY-zoom/v-rms-zoom-XY}\label{subfig:vrms-sgs-s4}}
  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S2.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/uv-av-zoom-XY}\label{subfig:uv-sgs-s2}}
  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S3.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-ds/XY-zoom/uv-av-zoom-XY}\label{subfig:uv-sgs-s3}}
  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S4.]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-vr/XY-zoom/uv-av-zoom-XY}\label{subfig:uv-sgs-s4}}
	\caption{Lateral view of RMS of time fluctuation
	of axial component of velocity, $u_{RMS}^{*}$, RMS 
	of time fluctuation of radial component of velocity, 
	$v_{RMS}^{*}$ and $\langle u^{*}v^{*}\rangle$ Reynolds 
	shear stress tensor component, for S2, S3 and S4.} 
	\label{fig:lat-u-v-uv-sgs}
\end{figure}
%
The profiles of $u^{*}_{RMS}$ at $X=2.5D$ obtained by S2, S3 and S4 are
in good agreement with the numerical reference, as one can observe in 
Fig.\ \ref{fig:prof-u-rms-sgs}. However, all simulations,
including the LES reference, fail to predict the peaks of $u^{*}_{RMS}$.
%
\begin{figure}[htb!]
  \centering
  \subfigure[$u^{*}_{RMS}$ - X=2.5D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/urms-2-5-sgs}}
  \subfigure[$u^{*}_{RMS}$ - X=5.0D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/urms-5-0-sgs}}
  \subfigure[$u^{*}_{RMS}$ - X=10D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/urms-10-0-sgs}}
  \subfigure[$u^{*}_{RMS}$ - X=15D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/urms-15-0-sgs}}
  \subfigure[$u^{*}_{RMS}$ - Centerline - Y=0 ; $0\leq X \leq 20D$ ]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/urms-centerline-sgs}}
  \subfigure[$u^{*}_{RMS}$ - Lipline - Y=0.5D ; $0\leq X \leq 20D$ ]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/urms-lipline-sgs}}
	\caption{Profiles of RMS of time fluctuation of axial 
	component of velocity, $u_{RMS}^{*}$, for S2, S3 and S4,
	at different positions within the computational domain.
	(\LARGE \textbf{--}\scriptsize), S2; 
	(\LARGE \textbf{-}\textbf{-}\scriptsize), S3;
	($\bigcirc$), S4; ($\square$), numerical data; 
	($\blacktriangle$), experimental data.}
	\label{fig:prof-u-rms-sgs}
\end{figure}
%
At $X=5.0D$ all three simulations have difficulties to predict the peaks 
of the profile. Nonetheless, the results are still in good agreement with
the literature. In the sequence, the profile of $u^{*}_{RMS}$ at $X=10.0D$
calculated by S2, S3 and S4 starts to diverge from the reference results.
Finally, at $X=15.0D$, all SGS closures, but the dynamic Smagorinsky model,
fail the predict the correct profile. S3 simulation have produced a profile 
of $u_{RMS}^{*}$ at $X=15.0D$ that is closer to the experimental data than
the numerical reference.

All three simulations have presented overestimated distributions of 
$u_{RMS}^{*}$ along the centerline. However, for $10D<X<15D$, the 
Vreman model correctly reproduces the magnitude of $u_{RMS}^{*}$.
All simulations performed in the present work have produced noisy 
distributions that diverge from the experimental data along the lipline.
One can notice that the numerical reference has also produced an 
overestimated distribution of $u_{RMS}^{*}$ at $X<10D$.


%\FloatBarrier

\subsubsection*{Root Mean Square Distribution of Time Fluctuations 
of Radial Velocity Component}

Effects of SGS modeling on the time fluctuation of the radial 
component of velocity are also compared with the reference data. 
Figures \ref{subfig:vrms-sgs-s2}, \ref{subfig:vrms-sgs-s3} and
\ref{subfig:vrms-sgs-s4} illustrate a lateral view of the 
distribution of $v_{RMS}^{*}$ computed by S2, S3 and S4, respectively. 
The SGS models does not significantly affect the distribution 
of $v_{RMS}^{*}$. All distributions calculated by S2, S3, S4 have 
shown similar behavior.

Four profiles of $v_{RMS}^{*}$ in the radial direction at $X=2.5D$, 
$X=5.0D$, $X=10.0D$ and $X=15.0D$ are presented in Fig.\ \ref{fig:prof-v-rms-sgs}. 
One can observe that, for $X\leq10.0D$, all the profiles calculated on S2, 
S3 and S4 are close to the reference. Moreover, the results of the static and the 
dynamic Smagorinsky models are in better agreement with experimental data than the LES
reference. At $X=15.0D$, all simulations performed in the current
work fail to predict the correct $v_{RMS}^{*}$ profile.

\FloatBarrier

%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[Lateral view of $v^{*}_{RMS}$ for S2.]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/XY-zoom/v-rms-zoom-XY}}
%  \subfigure[Lateral view of $v^{*}_{RMS}$ for S3.]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/XY-zoom/v-rms-zoom-XY}}
%  \subfigure[Lateral view of $v^{*}_{RMS}$ for S4.]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/XY-zoom/v-rms-zoom-XY}}
%	\caption{Lateral view of RMS of time fluctuation of radial 
%	component of velocity, $v_{RMS}^{*}$, for S2, S3 and S4.} 
%	\label{fig:lat-v-rms-sgs}
%\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure[$v^{*}_{RMS}$ - X=2.5D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/vrms-2-5-sgs}}
  \subfigure[$v^{*}_{RMS}$ - X=5.0D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/vrms-5-0-sgs}}
  \subfigure[$v^{*}_{RMS}$ - X=10D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/vrms-10-0-sgs}}
  \subfigure[$v^{*}_{RMS}$ - X=15D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/vrms-15-0-sgs}}
	\caption{Profiles of RMS of time fluctuation of radial 
	component of velocity, $v_{RMS}^{*}$, for S1 nd S2,
	at different positions within the computational domain.
	(\LARGE \textbf{--}\scriptsize), S2; 
	(\LARGE \textbf{-}\textbf{-}\scriptsize), S3;
	($\bigcirc$), S4; ($\square$), numerical data; 
	($\blacktriangle$), experimental data.}
	\label{fig:prof-v-rms-sgs}
\end{figure}
%





\subsubsection*{Component of Reynolds Stress Tensor}

Figures \ref{subfig:uv-sgs-s2}, \ref{subfig:uv-sgs-s3} and 
\ref{subfig:uv-sgs-s4} present lateral view and profiles of 
$\langle u^{*}v^{*}\rangle$ component of the Reynolds stress tensor 
computed using three different SGS models, respectively. One can 
observe that the simulation performed using different SGS models have 
produced very similar distributions of $\langle u^{*}v^{*} \rangle$ 
for the region where the mehs is refined. However, for $X>8.0D$ the 
properties calculated by the different SGS closures present different 
behavior. The spreading is not the same for S2, S3 and S4 where 
$X>8.0D$. Therefore, one can state that the static Smagorinsky, 
the dynamic Smagorinsky and the Vreman models react differently to 
the coarsening of the grid.

All numerical simulations performed in the present work have failed
to correct predict the profiles of $\langle u^{*}v^{*} \rangle$ 
presented in Fig.\ \ref{fig:prof-uv-av-sgs}. The peaks of the component
of the Reynolds stress tensor does not correlate with the reference 
results. However, one should notice that the LES performed by the 
reference has also presented difficulties to calculate the same peaks.
The cause of the issue could be related to an eventual lack of grid
points in the radial direction. In spite of that, more studies on the
subject are necessary in order to understand such behavior.
%
% Reynolds shear stress component of velocity
%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S2.]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/XY-zoom/uv-av-zoom-XY}}
%  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S3.]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/XY-zoom/uv-av-zoom-XY}}
%  \subfigure[Lateral view of $\langle u^{*}v^{*}\rangle$ for S4.]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/XY-zoom/uv-av-zoom-XY}}
%	\caption{Lateral view of the $\langle u^{*}v^{*}\rangle$ Reynolds 
%	shear stress tensor component, for S2, S3 and S4.} 
%	\label{fig:lat-uv-av-sgs}
%\end{figure}
%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=0.5D -- S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-0-5/uv-av-0-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=0.5D -- S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-0-5/uv-av-0-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=0.5D -- S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-0-5/uv-av-0-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=2.5D -- S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-2-5/uv-av-2-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=2.5D -- S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-2-5/uv-av-2-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=2.5D -- S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-2-5/uv-av-2-5-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=5.0D -- S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-5-0/uv-av-5-0-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=5.0D -- S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-5-0/uv-av-5-0-YZ}}
%  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=5.0D -- S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-5-0/uv-av-5-0-YZ}}
%	\caption{Frontal views of the $\langle u^{*}v^{*} \rangle$
%	Reynolds shear stress tensor component for S2, S3 and S4, 
%	at different positions along the axial coordinate. (\LARGE 
%	\textbf{-} \textbf{-}\normalsize) indicates the potential core 
%	of the jet, $U_{j}^{95\%}$.}
%	\label{fig:front-uv-av-sgs}
%\end{figure}
%
\begin{figure}[htb!]
  \centering
  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=2.5D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/uv-2-5-sgs}}
  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=5.0D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/uv-5-0-sgs}}
  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=10D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/uv-10-0-sgs}}
  \subfigure[$\langle u^{*}v^{*}\rangle$ - X=15D ; $-1.5D\leq Y\leq 1.5D$]
    {\includegraphics[width=0.45\textwidth]
	{sources/results/pictures/comparison/sgs/uv-15-0-sgs}}
	\caption{Profiles of the $\langle u^{*}v^{*} \rangle$ 
	Reynolds shear stress tensor component, for S2, S3 and S4, at 
    different positions within the computational domain.
	(\LARGE \textbf{--}\scriptsize), S2; 
	(\LARGE \textbf{-}\textbf{-}\scriptsize), S3;
	($\bigcirc$), S4; ($\square$), numerical data; 
	($\blacktriangle$), experimental data.}
	\label{fig:prof-uv-av-sgs}
\end{figure}

%\FloatBarrier

%\subsubsection*{Turbulent Kinectic Energy}
%
%Figures \ref{fig:lat-k-sgs} and \ref{fig:front-k-sgs} present
%lateral, detailed and frontal views of the turbulent kinetic
%energy distributions obtained by S2, S3 and S4. $k$ distributions
%can be interpretate as an property which accumulates the effects
%of the time fluctuation from all velocity components. One can notice 
%some differences on the $k$ distributions computed using different
%SGS models. The color scale indicates that the distribution of the
%turbulent kinetic energy calculated by the dynamic Smagorinsky model  
%is less intense when compared to the same distribution of $k$ computed
%by the static Smagorinsky and the Vreman models. S4 have reproduced
%a more spread distribution.
%
%%  Turbulent kinect energy
%%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$k$ - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/XY/k-av-XY}}
%  \subfigure[$k$ - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/XY-zoom/k-av-zoom-XY}}
%  \subfigure[$k$ - S3]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-ds/XY/k-av-XY}}
%  \subfigure[$k$ - S3]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-ds/XY-zoom/k-av-zoom-XY}}
%  \subfigure[$k$ - S4]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-vr/XY/k-av-XY}}
%  \subfigure[$k$ - S4]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-vr/XY-zoom/k-av-zoom-XY}}
%	\caption{Lateral view and detailed view of the
%	turbulent kinetic energy, $k$, for S2, S3 and S4.} 
%	\label{fig:lat-k-sgs}
%\end{figure}
%%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$k$ - X=0.5D -- S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-0-5/k-av-0-5-YZ}}
%  \subfigure[$k$ - X=0.5D -- S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-0-5/k-av-0-5-YZ}}
%  \subfigure[$k$ - X=0.5D -- S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-0-5/k-av-0-5-YZ}}
%  \subfigure[$k$ - X=2.5D -- S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-2-5/k-av-2-5-YZ}}
%  \subfigure[$k$ - X=2.5D -- S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-2-5/k-av-2-5-YZ}}
%  \subfigure[$k$ - X=2.5D -- S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-2-5/k-av-2-5-YZ}}
%  \subfigure[$k$ - X=5.0D -- S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-5-0/k-av-5-0-YZ}}
%  \subfigure[$k$ - X=5.0D -- S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-5-0/k-av-5-0-YZ}}
%  \subfigure[X=5.0D -- S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-5-0/k-av-5-0-YZ}}
%	\caption{Frontal views of the turbulent kinetic energy,
%	$k$, for S2, S3 and S4, at different positions along the axial 
%	coordinate. (\LARGE \textbf{-} \textbf{-}\normalsize) indicates 
%	the potential core 	of the jet, $U_{j}^{95\%}$.}
%	\label{fig:front-k-sgs}
%\end{figure}
%
%%\FloatBarrier
%
%\subsubsection*{Time Averaged Density}
%
%Figures \ref{fig:lat-rho-sgs} and \ref{fig:front-rho-sgs} presents
%the lateral, detailed and frontal views of the time averaged density
%calculated by S2, S3 and S4. The three turbulece models have reproduced
%similar $\langle\rho\rangle$ distributions near the entrance domain.
%The position of the shockwaves within the jet are the same for all 
%SGS models. Significative difference are observed only in the region 
%where the mesh does not present a good resolution.  
%
%%  Averaged Density
%%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$\langle\rho\rangle$ - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/XY/rho-av-XY}}
%  \subfigure[$\langle\rho\rangle$ - S2]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-cs/XY-zoom/rho-av-zoom-XY}}
%  \subfigure[$\langle\rho\rangle$ - S3]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-ds/XY/rho-av-XY}}
%  \subfigure[$\langle\rho\rangle$ - S3]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-ds/XY-zoom/rho-av-zoom-XY}}
%  \subfigure[$\langle\rho\rangle$ - S4]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-vr/XY/rho-av-XY}}
%  \subfigure[$\langle\rho\rangle$ - S4]
%    {\includegraphics[width=0.495\textwidth]
%	{sources/results/pictures/stat-vr/XY-zoom/rho-av-zoom-XY}}
%	\caption{Lateral view and detailed view of time averaged
%	density, $\langle\rho\rangle$, for S2, S3 and S4.} 
%	\label{fig:lat-rho-sgs}
%\end{figure}
%%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$\langle\rho\rangle$ - X=0.5D - S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-0-5/rho-av-0-5-YZ}}
%  \subfigure[$\langle\rho\rangle$ - X=0.5D - S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-0-5/rho-av-0-5-YZ}}
%  \subfigure[$\langle\rho\rangle$ - X=0.5D - S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-0-5/rho-av-0-5-YZ}}
%  \subfigure[$\langle\rho\rangle$ - X=2.5D - S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-2-5/rho-av-2-5-YZ}}
%  \subfigure[$\langle\rho\rangle$ - X=2.5D - S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-2-5/rho-av-2-5-YZ}}
%  \subfigure[$\langle\rho\rangle$ - X=2.5D - S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-2-5/rho-av-2-5-YZ}}
%  \subfigure[$\langle\rho\rangle$ - X=5.0D - S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-5-0/rho-av-5-0-YZ}}
%  \subfigure[$\langle\rho\rangle$ - X=5.0D - S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-5-0/rho-av-5-0-YZ}}
%  \subfigure[$\langle\rho\rangle$ - X=5.0D - S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-5-0/rho-av-5-0-YZ}}
%	\caption{Frontal views of the time averaged density,
%	$\langle\rho\rangle$, for S2, S3 and S4, at different positions 
%    along the axial coordinate. (\LARGE \textbf{-} \textbf{-}\normalsize) 
%	indicates the potential core of the jet, $U_{j}^{95\%}$.}
%	\label{fig:front-rho-sgs}
%\end{figure}
%
%\FloatBarrier
%

\subsubsection*{Time Averaged Eddy Viscosity}

The distribution of the eddy viscosity, $\mu_{t}$, is discussed 
in the current subsection. Figure \ref{fig:lat-mut-sgs} presents 
distributions of time averaged eddy viscosity calculated using 
different SGS models. All subgrid scale closures used in the present 
work, the static Smagorinsky \cite{Smagorinsky63,Lilly65,Lilly67}, 
the dynamic Smagorinsky \cite{Germano91,moin91} and the Vreman 
\cite{vreman2004} models, are dependent of the local mesh size 
by design. This characteristic is exposed on the lateral view 
of the flow presented in Fig.\ \ref{fig:lat-mut-sgs}. The SGS 
models are only acting in the region where mesh presents a low 
resolution. Near the entrance domain, where the computational 
grid is very refined, the eddy viscosity can be neglected. 

The remark goes in the same direction of the work of Li and Wang
\cite{Li15}, which indicates that SGS closures introduce numerical 
dissipation that can be used as a stabilizing mechanism. However, 
this numerical dissipation does not necessarily add more physics 
of the turbulence to the LES solution. Therefore, in the present 
work, the numerical truncation, which generates the dissipative 
characteristic of JAZzY solutions, have show to overcome the 
effects of the SGS modeling. The mesh need to be very fine in order
to achieve good results with second order spatial discretizations.
The grid refinement generates very small grid spacing. Consequently, 
the SGS models, which are strongly dependent on the filter width, does
not affect much the solution. A LES of compressible flow configurations
without the use of SGS closure would be welcome in order to complete 
such discussion.

%  Turbulent viscosity
%
\begin{figure}[htb!]
  \centering
  %\subfigure[$\langle\mu_{t}\rangle$ - S2]
  %  {\includegraphics[width=0.32\textwidth]
  %  {sources/results/pictures/stat-cs/XY/mut-av-XY}}
  \subfigure[$\langle\mu_{t}\rangle$ - S2]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-cs/XY-zoom/mut-av-zoom-XY}}
  %\subfigure[$\langle\mu_{t}\rangle$ - S3]
  %  {\includegraphics[width=0.32\textwidth]
  %  {sources/results/pictures/stat-ds/XY/mut-av-XY}}
  \subfigure[$\langle\mu_{t}\rangle$ - S3]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-ds/XY-zoom/mut-av-zoom-XY}}
  %\subfigure[$\langle\mu_{t}\rangle$ - S4]
  %  {\includegraphics[width=0.32\textwidth]
  %  {sources/results/pictures/stat-vr/XY/mut-av-XY}}
  \subfigure[$\langle\mu_{t}\rangle$ - S4]
    {\includegraphics[width=0.32\textwidth]
	{sources/results/pictures/stat-vr/XY-zoom/mut-av-zoom-XY}}
	\caption{Lateral view of time averaged eddy viscosity, 
	$\langle\mu_{t}\rangle$, for S2, S3 and S4.} 
	\label{fig:lat-mut-sgs}
\end{figure}
%
%\begin{figure}[htb!]
%  \centering
%  \subfigure[$\langle\mu_{t}\rangle$ - X=0.5D - S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-0-5/mut-av-0-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=0.5D - S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-0-5/mut-av-0-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=0.5D - S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-0-5/mut-av-0-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=2.5D - S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-2-5/mut-av-2-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=2.5D - S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-2-5/mut-av-2-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=2.5D - S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-2-5/mut-av-2-5-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=5.0D - S2]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-cs/YZ-5-0/mut-av-5-0-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=5.0D - S3]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-ds/YZ-5-0/mut-av-5-0-YZ}}
%  \subfigure[$\langle\mu_{t}\rangle$ - X=5.0D - S4]
%    {\includegraphics[width=0.32\textwidth]
%	{sources/results/pictures/stat-vr/YZ-5-0/mut-av-5-0-YZ}}
%	\caption{Frontal views of the time averaged eddy viscosity,
%	$\langle\mu_{t}\rangle$, for S1 and S2, at different positions along 
%	the axial coordinate. (\LARGE \textbf{-} \textbf{-}\normalsize) 
%	indicates the potential core of the jet, $U_{j}^{95\%}$.}
%	\label{fig:front-mut-sgs}
%\end{figure}
%
%\FloatBarrier

\subsubsection*{Power Spectral Density}

The power spectral density of $u^{*}$ is studied in the comparison 
of SGS modeling. Figure \ref{fig:psd-sgs} presents the PSD of $u^{*}$, 
in $dB$, as function of the Strouhal number for S2, S3 and S4. The same 
methodology used on the mesh refinement study is performed here. The 
signals of $u^{*}$ are collected from the sensors allocated in the 
computational domain. The signals of Fig.\ \ref{fig:psd-sgs} 
are shifted of -150{\bf dB} and -300{\bf dB} for $X=0.25D$ and $X=1.25$, 
respectively, in order to separate plots. 

One can observe that PSD signals along the lipline obtained using S2, S3 
and S4 have shown the same behavior. A small difference can be noticed for
higher Strouhal number for the first two sensors, located at $X=0.1D$ and
$X=0.25D$. Such remark is aligned to the same discussion performed about 
the eddy viscosity for different SGS models. The sensors are located 
in the region where the mesh present excellent resolution. Therefore,
the effects of the static Smagorinsky, the dynamic Smagorinsky and the 
Vreman models, which are strongly dependent on the filter width, can be 
neglected on $u^{*}$ for $X<1.25D$.
%
\begin{figure}[htb!]
  \centering
    {\includegraphics[width=0.56\textwidth]
	{sources/results/pictures/comparison/psd/psd-lipline-sgs}}
	\caption{Power spectral density of $u^{*}$ as function of the Strouhal
	number along the lipline of the jet.
    (\LARGE \textbf{--}\scriptsize), S2;
	(\LARGE {\color{red}\textbf{--}}\scriptsize), S3; 
	(\LARGE {\color{blue}\textbf{--}}\scriptsize), S4.
    A shift of -150 {\bf dB} and -300 {\bf dB} has been added to 
    the PSD in order to separate plots for $X=0.25D$ and $X=1.25D$, 
	respectively.}
	\label{fig:psd-sgs}
\end{figure}

% ------------------------------- section limit -------------------------------

\section{Concluding Remarks}

The current work is the study on effects of different 
subgrid scales models on perfectly expanded supersonic jet 
flow configurations using centered second-order spatial 
discretization. A formulation based on the the System I set 
of equations is used in the present work. The time integration 
is performed using a five-steps second order Runge-Kutta scheme.
Four large eddy simulations of compressible jet flows are performed 
in the present research using two different mesh configurations 
an three different subgrid scale models. Their effects
on the large eddy simulation solution are compared and discussed.

The mesh refinement study has indicated that in the region 
where the grid presents high resolution, the simulations
are in good agreement with experimental and numerical 
references. For the mesh with 14 million points the simulation 
has produced good results for $X<2.5D$ and $-1.5D<Y<0.5D$.
For the other mesh, with 50 million points, the simulations
provided good agreement with the literature for $X<5.0D$ and 
$-1.5D<Y<0.5D$. The eddy viscosity, calculated by the static
Smagorinsky model, presents very low levels in the region 
where the results have good correlation with the results of
the literature.

The refined grid used on the mesh refinement study, mesh B,
is used for the comparison of SGS models effects on the 
results of large eddy simulations. Three compressible jet
flow simulations are performed using the classic Smagorinsky
model \cite{Smagorinsky63,Lilly65,Lilly67}, the dynamic 
Smagorinsky model \cite{Germano91,moin91} and the Vreman model
\cite{vreman2004}. All three simulations presented similar 
behavior. Results presented good agreement with the reference 
for $X<5.0D$. In the region where the grid is very fine and 
the results correlates well with the literature, the eddy 
viscosity, provided by the SGS model, is very low values. 
The reason is related to the fact that the SGS closures used 
in the current work are strongly dependent of the filter width, 
which is proportional to the local mesh size. 

The numerical results indicated that it is possible to achieve
good results using second-order spatial discretization. The
mesh ought be well resolved in order to overcome the truncation 
errors from the low order numerical scheme. Very fine meshes 
originates very small filter width. Consequently, the effects 
of the eddy viscosity calculated by the SGS models on the
solution become unimportant. The work of Li and Wang \cite{Li15} 
have presented similar conclusions for simplified problems.
The authors indicate that SGS closures introduce numerical 
dissipation that can be used as a stabilizing mechanism. 
However, this numerical dissipation does not necessarily add 
more physics of the turbulence to the LES solution. Simulations 
without the use of any SGS model are welcome and could reinforce 
the argument.

% ------------------------------- section limit -------------------------------

\section*{Acknowledgments}

The authors gratefully acknowledge the partial support for this research provided by
Conselho Nacional de Desenvolvimento Cient\'ifico e Tecnol\'ogico, CNPq, under the
Research Grants No.\ 309985/2013-7, No.\ 400844/2014-1 and No.\ 443839/2014-0\@.
The authors are also indebted to the partial financial support received from 
Funda\c{c}\~{a}o de Amparo \`{a} Pesquisa do Estado de S\~{a}o Paulo, FAPESP, 
under the Research Grants No.\ 2008/57866-1, No.\ 2013/07375-0 and No.\ 2013/21535-0. 





==> sources/turb_mod/turb_mod.tex <==
\section{Subgrid Scale Modeling} \label{ch:turb_mod}

The SGS terms presented in Eqs.\ \eqref{eq:les_qdm} and
\eqref{eq:les_energy} cannot be directly calculated. 
Subgrid scale models are necessary in order to close 
the LES set of equations. The closure models presented 
here are based on homogeneous turbulence theory, 
which is usually developed in spectral space as an 
atempt to quantify the interaction between the different 
scales of turbulence.

\subsection{Subgrid Scale Viscosity}

The SGS stress tensor is here calculated using
the concept that the forward energy cascade is analogous 
to the molecular mechanisms represented by the molecular 
viscosity whose mathematical structure follows the Boussinesq 
hypothesis \cite{Boussinesq1877} to explicitly introduce 
the subgrid scale viscosity, $\mu_{sgs}$,
%
\begin{equation}
\sigma_{ij}^{d} = \sigma_{ij} - \frac{1}{3} \delta_{ij} \sigma_{kk} = 
-2 \mu_{sgs} \left( \check{S}_{ij} - \frac{1}{3} \check{S}_{kk} \right) \, \mbox{.}
\end{equation}
%
The isotropic portion of the SGS stress tensor is 
generally weak with respect to the thermodynamic 
pressure \cite{Erlebacher92}. Therefore, $\sigma_{kk}$
is neglected in the present paper and $\sigma_{ij}$ 
is written as
%
\begin{equation}
\sigma_{ij} = -2 \mu_{sgs} \left( \check{S}_{ij} 
- \frac{1}{3} \check{S}_{kk} \right) \, \mbox{.}
\end{equation}
%
The Smagorinsky model \cite{Smagorinsky63, Lilly65} is used to 
calculate the SGS viscosity and it is given by 
%
\begin{equation}
	\mu_{sgs} = \overline{\rho} \left( C_{s} \Delta \right)^{2}  
\left( 2 \check{S}_{ij} \check{S}_{ij} \right)^{\frac{1}{2}}
\, \mbox{,}
\end{equation}
%
and $C_{s}$ is the Smagorinsky constant. Several 
attempts can be found in the literature regarding the evaluation
of the Smagorinsky constant. The value of this constant is adjusted to 
improve the results of different flow configurations. In pratical terms, 
the Smagorinsky constant assumes value ranging from 0.1 to 0.2 depending on the 
flow. The present work uses $C_{s}=0.18$ as suggested by Lilly
\cite{Lilly67}.

\subsection{Subgrid Scale Modeling of the Energy Equation}

Some of the SGS terms within the System I formulation 
\cite{Vreman1995} are not directly computable. Therefore, modeling 
is applied in order to close the system. Several papers in the literature
\cite{Garnier09,Erlebacher92,moin91,Martin00,lenormand2000,coleman1995} 
evaluate the relevance of the SGS terms on different applications. 
The LES community commonly uses the hypothesis of Eidson 
\cite{eidson85}, which assumes that the energy transfer from the 
resolved scales is proportional to the gradient of the resolved 
temperature \cite{Garnier09}. The proportionality coefficient 
is the subgrid scale conductivity, $\kappa_{sgs}$, which is 
linked to the subgrid scale viscosity through the relation 
%
\begin{equation}
	\kappa_{sgs} = \frac{\overline{\rho}\, \nu_{sgs}\, C_{p}}{{Pr}_{sgs}} 
	\, \mbox{,}
\end{equation}
%
in which $Pr_{sgs}$ is the SGS Prandtl number. The eddy-damped 
quasi-normal Markovian (EDQNM) theory \cite{lesieur08} considers 
$Pr_{sgs}=0.6$. In the present work, the concept of SGS conductivity, 
$\kappa_{sgs}$, is used in order to model $B_{1} + B_{2}$, {\em i.e.}, 
%
\begin{equation}
	B_{1} + B_{2} = -\frac{\partial}{\partial x_{j}} 
	\left( \kappa_{sgs} \frac{\partial \tilde{T}}{\partial x_{j}} \right) 
	\, \mbox{,}
\end{equation}
%
Following the work of Larcheveque \cite{larcheveque03}, $B_{4}$, $B_{5}$, 
$B_{6}$ and $B_{7}$ are neglected in the present paper.


\subsection{Shear-Stress Tensor Modeling}

The difference between the shear-stress tensors at the right-hand side of the 
momentum equations is neglected in the present work,
%
\begin{equation}
    \overline{\tau_{ij}} - \check{\tau}_{ij} = 0
\end{equation}

